Analysis and Evaluation of Non-Blocking Interpolation Search Trees

We start by summarizing the recently proposed implementation of the first non-blocking concurrent interpolation search tree (C-IST) data structure. We then analyze the individual operations of the C-IST, and show that they are correct and linearizable. We furthermore show that lookup (and several other non-destructive operations) are wait-free, and that the insert and delete operations are lock-free. We continue by showing that the C-IST has the following properties. For arbitrary key distributions, this data structure ensures worst-case $O(\log n + p)$ amortized time for search, insertion and deletion traversals. When the input key distributions are smooth, lookups run in expected $O(\log \log n + p)$ time, and insertion and deletion run in expected amortized $O(\log \log n + p)$ time, where $p$ is a bound on the number of threads. Finally, we present an extended experimental evaluation of the non-blocking IST performance.

==> experiments/old-old-i7-4930mx/lookup.ordered.tex <==
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=5.0cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=$size$,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=-90,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=-90,
  },
  ytick={128, 256, 384, 512, 640},
  ybar=0.1pt,
  bar width=6pt,
  x=1.77cm,
  ymin=0,
  ymax=800,
  x,
  axis on top,
  xtick=data,
  symbolic x coords={
    1000k, 2000k, 4000k, 10000k
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=3,
    at={(0.90, 0.98)},
    anchor=north east,
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1000k, 66.50996244999999) += (0,5.579758837663277) -= (0,5.579758837663277)
(2000k, 137.40313264999998) += (0,12.896686664025875) -= (0,12.896686664025875)
(4000k, 228.27578500000004) += (0,17.207750014526074) -= (0,17.207750014526074)
(10000k, 266.55235315) += (0,61.96389152705548) -= (0,61.96389152705548)
};
\addlegendentry{IST}
\node[above] at ($(axis cs:1000k, 66.5)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:2000k, 137.4)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:4000k, 228.27)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:10000k, 266.55)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1000k, 74.7965465) += (0,1.535314825899124) -= (0,1.535314825899124)
(2000k, 171.84619025) += (0,3.581281066284745) -= (0,3.581281066284745)
(4000k, 321.5009102) += (0,17.567784823457366) -= (0,17.567784823457366)
(10000k, 322.5780262) += (0,8.572085564542537) -= (0,8.572085564542537)
};
\addlegendentry{Btree}
\node[above] at ($(axis cs:1000k, 74.79)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.1\times$}}};
\node[above] at ($(axis cs:2000k, 171.84)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.2\times$}}};
\node[above] at ($(axis cs:4000k, 321.5)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.4\times$}}};
\node[above] at ($(axis cs:10000k, 322.57)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.2\times$}}};

\addplot[
  fill={rgb:red,5;green,1;blue,1},
    postaction={
      pattern color=white,
      pattern=north west lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1000k, 110.88980395000002) += (0,2.66303765435184) -= (0,2.66303765435184)
(2000k, 235.97615209999998) += (0,7.461923705111844) -= (0,7.461923705111844)
(4000k, 484.76907309999996) += (0,18.899945508000986) -= (0,18.899945508000986)
(10000k, 505.74930595000006) += (0,15.342245345050822) -= (0,15.342245345050822)
};
\addlegendentry{skiplist}
\node[above] at ($(axis cs:1000k, 110.88)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.6\times$}}};
\node[above] at ($(axis cs:2000k, 235.97)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.7\times$}}};
\node[above] at ($(axis cs:4000k, 484.76)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$2.1\times$}}};
\node[above] at ($(axis cs:10000k, 505.74)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.8\times$}}};

\node[anchor=south west] at (rel axis cs:0,0) [xshift=-14mm,yshift=-6mm]
{i7-4930mx};
\legend{}
\end{axis}
\end{tikzpicture}

==> experiments/old-old-i7-4930mx/lookup.par.6.shuffled.4M.tex <==
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=5.0cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=$\#proc$,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=-90,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=-90,
  },
  ytick={256, 512, 768, 1,024, 1,280, 1,536, 1,792, 2,048},
  ybar=0.1pt,
  bar width=6pt,
  x=0.44cm,
  ymin=0,
  ymax=2457.6,
  x,
  axis on top,
  xtick=data,
  symbolic x coords={
    6
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=3,
    at={(0.90, 0.98)},
    anchor=north east,
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(6, 308.63209500000005) += (0,15.447116970822421) -= (0,15.447116970822421)
};
\addlegendentry{IST}
\node[above] at ($(axis cs:6, 308.63)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(6, 768.7883904) += (0,12.870897881047387) -= (0,12.870897881047387)
};
\addlegendentry{Btree}
\node[above] at ($(axis cs:6, 768.78)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$2.4\times$}}};

\addplot[
  fill={rgb:red,5;green,1;blue,1},
    postaction={
      pattern color=white,
      pattern=north west lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(6, 1270.6630754000003) += (0,4.504182557810987) -= (0,4.504182557810987)
};
\addlegendentry{skiplist}
\node[above] at ($(axis cs:6, 1270.66)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$4.1\times$}}};

\node[anchor=south west] at (rel axis cs:0,0) [xshift=-3mm,yshift=-6mm]
{amd64};
\legend{}
\end{axis}
\end{tikzpicture}

==> experiments/old-old-i7-4930mx/lookup.par.shuffled.400k.tex <==
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=5.0cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=$\#proc$,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=-90,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=-90,
  },
  ytick={64, 128, 192, 256, 320, 384, 448, 512},
  ybar=0.1pt,
  bar width=6pt,
  x=1.77cm,
  ymin=0,
  ymax=614.4,
  x,
  axis on top,
  xtick=data,
  symbolic x coords={
    1, 2, 4, 8
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=3,
    at={(0.90, 0.98)},
    anchor=north east,
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1, 82.60833075000002) += (0,6.352634747150955) -= (0,6.352634747150955)
(2, 42.192539599999996) += (0,1.9835662715827882) -= (0,1.9835662715827882)
(4, 23.892591449999998) += (0,3.155748390533512) -= (0,3.155748390533512)
(8, 15.822654750000002) += (0,1.68202640376285) -= (0,1.68202640376285)
};
\addlegendentry{IST}
\node[above] at ($(axis cs:1, 82.6)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:2, 42.19)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:4, 23.89)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:8, 15.82)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1, 138.69717755000005) += (0,2.484799853622713) -= (0,2.484799853622713)
(2, 73.36082639999998) += (0,0.9342914805808402) -= (0,0.9342914805808402)
(4, 42.189458000000016) += (0,1.0984688093306978) -= (0,1.0984688093306978)
(8, 26.95433275) += (0,6.163337403143883) -= (0,6.163337403143883)
};
\addlegendentry{Btree}
\node[above] at ($(axis cs:1, 138.69)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.6\times$}}};
\node[above] at ($(axis cs:2, 73.36)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.7\times$}}};
\node[above] at ($(axis cs:4, 42.18)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.7\times$}}};
\node[above] at ($(axis cs:8, 26.95)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.7\times$}}};

\addplot[
  fill={rgb:red,5;green,1;blue,1},
    postaction={
      pattern color=white,
      pattern=north west lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1, 296.7559449) += (0,4.1787933518095315) -= (0,4.1787933518095315)
(2, 154.7161552) += (0,3.801517370602146) -= (0,3.801517370602146)
(4, 88.99213445000001) += (0,1.6373855838808848) -= (0,1.6373855838808848)
(8, 52.68202114999999) += (0,3.0282762445212175) -= (0,3.0282762445212175)
};
\addlegendentry{skiplist}
\node[above] at ($(axis cs:1, 296.75)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$3.5\times$}}};
\node[above] at ($(axis cs:2, 154.71)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$3.6\times$}}};
\node[above] at ($(axis cs:4, 88.99)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$3.7\times$}}};
\node[above] at ($(axis cs:8, 52.68)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$3.3\times$}}};

\node[anchor=south west] at (rel axis cs:0,0) [xshift=-14mm,yshift=-6mm]
{i7-4930mx};
\legend{}
\end{axis}
\end{tikzpicture}

==> experiments/old-old-i7-4930mx/lookup.par.shuffled.tex <==
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=5.0cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=$\#proc$,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=-90,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=-90,
  },
  ytick={256, 512, 768, 1024, 1280, 1536, 1792},
  ybar=0.1pt,
  bar width=6pt,
  x=1.77cm,
  ymin=0,
  ymax=2057.6,
  x,
  axis on top,
  xtick=data,
  symbolic x coords={
    1, 2, 4, 8
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=3,
    at={(0.90, 0.98)},
    anchor=north east,
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1, 1180.9500724000002) += (0,22.923620596702442) -= (0,22.923620596702442)
(2, 666.85129265) += (0,77.94710042771204) -= (0,77.94710042771204)
(4, 304.48951935) += (0,6.409932696183495) -= (0,6.409932696183495)
(8, 208.35644675000003) += (0,7.103590472252058) -= (0,7.103590472252058)
};
\addlegendentry{IST}
\node[above] at ($(axis cs:1, 1180.95)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:2, 666.85)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:4, 304.48)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:8, 208.35)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\node[anchor=south west] at (rel axis cs:0,0) [xshift=-14mm,yshift=-6mm]
{i7-4930mx};
\legend{}
\end{axis}
\end{tikzpicture}

==> experiments/old-old-i7-4930mx/lookup.shuffled.tex <==
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=5.0cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$ms$,
  xlabel=$size$,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-8,
    yshift=-12,
    anchor=south,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=-90,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=-90,
  },
  ytick={4096, 8192, 12288, 16384, 20480},
  ybar=0.1pt,
  bar width=6pt,
  x=1.77cm,
  ymin=0,
  ymax=20321.6,
  x,
  axis on top,
  xtick=data,
  symbolic x coords={
    1000k, 2000k, 4000k, 10000k
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=3,
    at={(0.90, 0.98)},
    anchor=north east,
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1000k, 310.8853371000001) += (0,43.29127166949444) -= (0,43.29127166949444)
(2000k, 552.9767691999999) += (0,15.86945484855008) -= (0,15.86945484855008)
(4000k, 1216.864816) += (0,23.239774795960944) -= (0,23.239774795960944)
(10000k, 3308.5538199999996) += (0,159.0445567427154) -= (0,159.0445567427154)
};
\addlegendentry{IST}
\node[above] at ($(axis cs:1000k, 310.88)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:2000k, 552.97)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:4000k, 1216.86)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};
\node[above] at ($(axis cs:10000k, 3308.55)$) [xshift=-1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.0\times$}}};

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1000k, 447.1757620499999) += (0,3.1131000069321972) -= (0,3.1131000069321972)
(2000k, 1123.0471525000003) += (0,8.171172658242655) -= (0,8.171172658242655)
(4000k, 2619.0585014000003) += (0,226.91629789875947) -= (0,226.91629789875947)
(10000k, 5545.426286700001) += (0,951.3874794855024) -= (0,951.3874794855024)
};
\addlegendentry{Btree}
\node[above] at ($(axis cs:1000k, 447.17)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.4\times$}}};
\node[above] at ($(axis cs:2000k, 1123.04)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$2.0\times$}}};
\node[above] at ($(axis cs:4000k, 2619.05)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$2.1\times$}}};
\node[above] at ($(axis cs:10000k, 5545.42)$) [xshift=0.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$1.6\times$}}};

\addplot[
  fill={rgb:red,5;green,1;blue,1},
    postaction={
      pattern color=white,
      pattern=north west lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1000k, 991.9616567999998) += (0,38.64042562274706) -= (0,38.64042562274706)
(2000k, 2387.88326305) += (0,47.54845297025478) -= (0,47.54845297025478)
(4000k, 5402.63734555) += (0,352.3814802959659) -= (0,352.3814802959659)
(10000k, 17471.282968849995) += (0,1615.403265354643) -= (0,1615.403265354643)
};
\addlegendentry{skiplist}
\node[above] at ($(axis cs:1000k, 991.96)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$3.1\times$}}};
\node[above] at ($(axis cs:2000k, 2387.88)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$4.3\times$}}};
\node[above] at ($(axis cs:4000k, 5402.63)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$4.4\times$}}};
\node[above] at ($(axis cs:10000k, 17471.28)$) [xshift=1.0*\pgfkeysvalueof{/pgf/bar width}]
{\rotatebox{-90}{\scriptsize{$5.2\times$}}};

\node[anchor=south west] at (rel axis cs:0,0) [xshift=-14mm,yshift=-6mm]
{i7-4930mx};
\legend{}
\end{axis}
\end{tikzpicture}

==> experiments/old-xeon-gold-6150-x4/llc.tex <==
\begin{tikzpicture}[scale=0.78]
  \begin{axis}[
  height=5.0cm,
  every axis plot post/.style={/pgf/number format/fixed},
  ylabel=$miss/lookup$,
  xlabel=$size$,
  grid=both,
  every axis y label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=-0,
    yshift=-30,
    anchor=south,
    rotate=-90,
  },
  every axis x label/.style={
    at={(ticklabel* cs:1.05)},
    xshift=12,
    yshift=-10,
    anchor=north,
    rotate=-90,
  },
  scaled y ticks=false,
  yticklabel style={
    /pgf/number format/fixed,
  },
  xticklabel style={
    rotate=0,
  },
  ytick={4, 8, 12, 16, 20, 24, 28, 32},
  ybar=0.1pt,
  bar width=7pt,
  x=1.35cm,
  ymin=0,
  ymax=38,
  x,
  axis on top,
  xtick=data,
  symbolic x coords={
    1M, 10M, 100M, 1B
  },
  % restrict y to domain*=0:75,
  visualization depends on=rawy\as\rawy,
  axis lines*=left,
  clip=false,
  legend style={
    legend columns=3,
    at={(0.90, 0.98)},
    anchor=north east,
  },
  draw opacity=0.4,
  major grid style={
    draw opacity=0.3,
  },
]
    
\addplot[
  fill={rgb:red,1;green,4;blue,5},
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1M, 0.09)
(10M, 6.0)
(100M, 9.8)
(1B, 13.1)
};
\addlegendentry{IST}

\addplot[
  fill={rgb:red,1;green,3;blue,1},
    postaction={
      pattern color=white,
      pattern=north east lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1M, 1.5)
(10M, 6.6)
(100M, 11.8)
(1B, 19.0)
};

\addplot[
  fill={rgb:red,5;green,1;blue,1},
    postaction={
      pattern color=white,
      pattern=north west lines,
    },
  error bars/.cd,
  error bar style=red,
  y dir=both,
  y explicit,
]
plot coordinates {
(1M, 3.5)
(10M, 10.9)
(100M, 20.5)
(1B, 33.2)
};
\addlegendentry{skiplist}

\node[anchor=south west] at (rel axis cs:0,0) [xshift=-8mm,yshift=-9mm]
{};
\legend{}
\end{axis}
\end{tikzpicture}

==> parts/abstract.tex <==
% !TEX root = ../main.tex

\begin{abstract}
  Balanced search trees typically use key comparisons to guide their operations,
  and achieve logarithmic running time.
  By relying on numerical properties of the keys,
  \emph{interpolation search} achieves lower search complexity and better performance.
  Although interpolation-based data structures were investigated in the past,
  their non-blocking concurrent variants have received very little attention so far.

  In this paper, we propose the first non-blocking implementation
  of the classic interpolation search tree (IST) data structure.
  For arbitrary key distributions,
  the data structure ensures worst-case $O(\log n + p)$ amortized time
  for search, insertion and deletion traversals.
  When the input key distributions are \emph{smooth},
  lookups run in expected $O(\log \log n + p)$ time,
  and insertion and deletion run in expected amortized $O(\log \log n + p)$ time, 
  where $p$ is a bound on the number of threads.
  To improve the scalability of concurrent insertion and deletion,
  we propose a novel parallel rebuilding technique, which should be of independent interest. 

  We evaluate whether the theoretical improvements translate to practice by implementing the 
  concurrent interpolation search tree, and benchmarking it on uniform and
  non-uniform key distributions, for dataset sizes in the millions to billions of keys. 
  Relative to the state-of-the-art concurrent data structures,
  the concurrent interpolation search tree achieves performance improvements
  of up to $15 \%$ under high update rates,
  and of up to $50\%$ under moderate update rates.
  Further, ISTs exhibit up to $2\times$ less cache-misses,
  and consume $1.2-2.6\times$ less memory compared to the next best alternative
  on typical dataset sizes. 
  We find that the results are surprisingly robust to distributional skew,
  which suggests that our data structure can be a promising alternative to
  classic concurrent search structures. 

\end{abstract}


==> parts/algorithm.tex <==
% !TEX root = ../main.tex

\section{Concurrent Interpolation Search Tree}
\label{sec:algorithm}

\subsection{Examples and Overview}
\label{sec:examples}

We illustrate how concurrent interpolation search trees work using several examples.
Examine the first tree in the following figure.
Each inner node consists of a set of $d$ pointers to child nodes,
and $d - 1$ keys that are used to drive the search.
We say that the node's \emph{degree} is $d$.
The top node usually has the highest degree,
and the degree of a node decreases as it gets deeper in the tree
(explained precisely below).
The tree is \emph{external}, meaning that the keys are stored in the leaf nodes.
The illustration shows a subset of nodes --
the missing nodes are represented with $\cdots$ symbols.

\begin{center}
\includegraphics[scale=0.27]{figures/insert-example-1.pdf}
\end{center}

Consider the task of inserting a key $k_m$,
such that $k_j < k_m < k_l$,
where $k_j$ and $k_l$ are existing keys in the tree.
%\trevor{
%This task seems under specified.
%Do we want to say $k_j < k_m < k_n$ for some other $k_n$?
%}
The figure shows a tree in which $k_j$ is contained in a leaf node on the bottom.
Insertion finds the leaf corresponding to $k_j$,
such that $k_m$ is the successor of $k_j$,
and then allocates a new inner node that holds both $k_j$ and $k_m$.
Finally, the old pointer in the parent is atomically changed
with a §CAS§ instruction to point to the new node.

Without rebalancing,
the tree can become arbitrarily deep.
Therefore, insertion must periodically rebalance parts of the tree.
The following figure shows the tree after inserting an additional key $k_n$,
such that $k_i < k_j < k_m < k_n$.
The subtree at the bottom, which contains the keys $k_i$, $k_j$, $k_m$ and $k_n$,
is sufficiently imbalanced, and it should be replaced with a more balanced tree.
Rebalancing creates a new subtree that contains the same set of keys.
%\trevor{
%Here, we're talking about rebuilding for the first time.
%Should we explain that we rebuild?
%}
After rebalancing,
the subtree consists of a single inner node of degree $4$,
as shown on the right.
Note that deletions also periodically rebalance the subtrees.
%\trevor{
%Should we briefly mention that deletions also rebalance? In parentheses?
%``(Deletions also periodically rebuild unbalanced subtrees.)''
%}

\begin{center}
\includegraphics[scale=0.27]{figures/insert-example-2.pdf}
\end{center}

There are several challenges with this approach.
First, concurrent modifications and rebalancing
must correctly synchronize so that all operations remain non-blocking,
while searches remain wait-free.
%\trevor{
%Should we additionally mention that we want searches to be able
%to ignore ongoing rebalancing so they are ultra fast?
%``(Additionally, it is desirable to allow searches to ignore ongoing rebuilding.)''
%}
% Second, it must be possible to track the amount of imbalance
% in each subtree without causing too much contention.
% Finally, the algorithm for deciding when to rebalance
% must be designed so that operations run in $O(\log \log n)$ time
% when the probability distribution of the input keys is smooth \cite{IST}.
%Finally, rebalancing criteria must be picked in a way such that,
%when the probability distribution of the input keys is sufficiently smooth,
%operations run in amortized $O(\log \log n)$ time.
%\trevor{
%perhaps ``Finally, the algorithm for deciding when and how to rebuild
%must be designed so that, when''?
%}
% NEW VERSION BELOW
Second, the rebalancing of any subtree
must not compromise the scalability of the other operations.
Finally, concurrent rebalancing must,
when the probability distribution of the input keys is smooth~\cite{IST},
ensure that the operations run in amortized $O(\log \log n)$ time.


\subsection{Data Types}
\label{sec:data-types}

The concurrent interpolation search tree consists of the data types
shown in Figure~\ref{algo:data-types}.
The §IST§ data type represents the interpolation search tree
with the single member §root§, which points to the root node.
% For convenience, the root node always has degree $d$.
Initially, the root node points to an empty leaf node, whose type is §Empty§.
The §Single§ data type represents a leaf node with a single key and an associated value,
and the §Inner§ data type represents inner nodes,
as illustrated on the right of Figure~\ref{algo:data-types}.

\begin{figure*}[]
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[numbers=none]
struct IST is
  root: Node

struct Single: Node is
  key: KeyType
  val: ValType
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[numbers=none]
struct Inner: Node is
  initSize: int
  degree: int
  keys: KeyType[]
  children: Node[]
  status: [int, bool, bool]
  count: int
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[numbers=none]
struct Empty: Node is

struct Rebuild: Node is
  target: Inner
  parent: Inner
  index: int
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.24\textwidth}
\vspace{0.1cm}
\includegraphics[scale=0.21]{figures/data-types.pdf}
\end{minipage}
\vspace{-7mm}
\caption{Data Types}
\label{algo:data-types}
\end{figure*}

In addition to holding the search keys,
and the pointers to the child nodes,
the §Inner§ data type contains the node's §degree§,
and a field called §initSize§,
which contains the number of keys
that were in the corresponding subtree when this node was created.
Apart from the child pointers, these fields are set on creation,
and not subsequently modified.

§Inner§ also contains two volatile fields,
§count§ and §status§, which are used to coordinate rebuilding.
The §count§ field holds the number of updates that were performed
in the subtree rooted at this node since it was created.
The §status§ field consists of an integer and two booleans --
it is initially zero,
and then changes to a non-zero value to indicate
that this node will be replaced during a rebuilding operation.

The §Rebuild§ data type contains information about a subtree-rebuilding operation.
It contains a pointer called §target§ to the root of the subtree to rebuild,
a pointer to its §parent§,
and the §index§ of the §target§ in the §parent§ node's array of child pointers.
The §status§ field and the §Rebuild§ type
are further explained in Section \ref{sec:partial-rebuild}.

To perform correctly, IST operations must maintain certain invariants --
informally, these invariants state that there must be a unique, acyclic path to any key,
and that the nodes cover disjoint key intervals.
They are formally defined below.

\begin{invariant}[Key presence]
\label{inv:presence}
  For any key §k§ reachable in the IST §I§,
  there exists exactly one path of the form §I§
  $\overset{\texttt{root}}{\rightarrow}$ §n§$_0$
  $\overset{\texttt{children[i$_0$]}}{\rightarrow}$
  $(§n§_1 \enskip | \enskip §r§_1 \overset{\texttt{target}}{\rightarrow} §n§_1)$
  $\overset{\texttt{children[i$_1$]}}{\rightarrow}$
  $\ldots$
  $\overset{\texttt{children[i$_{m-1}$]}}{\rightarrow}$
  $(§n§_m \enskip | \enskip §r§_m \overset{\texttt{target}}{\rightarrow} §n§_m)$,
  where §n§$_m$ holds the key §k§, §r§$_m$ is a §Rebuild§ node,
  and $|$ is a choice between two patterns.
\end{invariant}

% \begin{invariant}[Key absence]
% \label{inv:absence}
%   There does not exist any path that starts with §I.root§
%   and ends with a leaf that holds the key §k§,
% \end{invariant}

\begin{definition}[Cover]
\label{def:cover}
A root node §n§
\emph{covers} the interval $\langle -\infty, \infty \rangle$.
Given an inner node §n§ of degree $d$ that covers the interval $[ a, b \rangle$,
and holds the keys $k_0, k_1, \ldots, k_{d-2}$ in its §keys§ array,
its child §n.children[i]§ covers the interval $[ k_{i-1}, k_i \rangle$,
where we define $k_{-1} = a$ and $k_{d-1} = b$.
\end{definition}

\begin{definition}[Content]
A node §n§ \emph{contains} a key §k§ if and only if
the path from the root of the IST §I§ to the leaf with the key §k§
contains the node §n§.
An IST §I§ \emph{contains} a key §k§ if and only if the §root§ contains the key §k§.
\end{definition}

\begin{invariant}[Search tree]
\label{inv:search}
If a node §n§ covers $[ a, b \rangle$ and contains a key §k§,
then §k§ $\in [ a, b \rangle$.
\end{invariant}

\begin{invariant}[Acyclicity]
\label{inv:acyclicity}
There are no cycles in the interpolation search tree.
\end{invariant}

\begin{definition}[Has-key]
\label{def:has-key}
Relation $\haskey(§I§, k)$ holds if and only if §I§ satisfies the invariants,
and contains the key $k$.
\end{definition}

In the interpolation search tree,
the degree $d$ of a node with cardinality $n$ is $\Theta(\sqrt{n})$.
In an \emph{ideal IST},
the degree of a node with cardinality $n$
is either $\floor{\sqrt{n}}$ or $\ceil{\sqrt{n}}$,
and the number of keys in each of the node's subtrees is $\Theta(\sqrt{n})$,
more specifically, either $\floor{\sqrt{n}}$ or $\ceil{\sqrt{n}}$.
This ensures the $O(\log \log n)$ depth bound.
An example of an ideal IST is shown below --
the root has a degree $\Theta(\sqrt{n})$,
its children have the degree $\Theta(\sqrt[4]{n})$,
its grandchildren have the degree $\Theta(\sqrt[8]{n})$ and so on.
The interpolation search tree will generally not be ideal
after a sequence of insertion and deletion operations,
but its subtrees are ideal ISTs immediately after they get rebuilt.

\begin{center}
\includegraphics[scale=0.24]{figures/ideal.pdf}
\end{center}


\subsection{Insertion and Deletion}
\label{sec:insertion-deletion}

%\trevor{
%What do we do if the key is already present?
%Even if it's very simple,
%the pseudocode doesn't handle this, and I don't talk about it (yet).
%}

As illustrated in Section \ref{sec:examples},
an insertion searches the tree for a §Single§ or §Empty§ node,
and then replaces this node with one or two new nodes.
An §Empty§ node is replaced with a new §Single§ node that contains the new key,
and a §Single§ node is replaced with an inner node.

To track the amount of imbalance in each subtree,
the standard IST increments the §count§ for all the inner nodes that lead to that leaf,
whenever a key is inserted or deleted at that leaf \cite{IST}.
Once some §count§ reaches a threshold, the corresponding subtree is rebuilt.
Our C-IST implementation avoids contention at the root
by using a scalable, quiescently-consistent multicounter~\cite{ABKLN} at the root.

Once rebalancing is triggered,
subsequent insertions and deletions in the corresponding subtree must fail,
and help complete the rebalancing before retrying.
To ensure this, the rebalancing sets the §status§ field of all the nodes
of the target subtree.
An insertion atomically checks the §status§ field of an inner node
while replacing a child of the inner node.
We accomplish this with an atomic double-compare-single-swap (§DCSS§) primitive,
which takes two addresses,
two corresponding expected values, and one new value as arguments,
and behaves like a §CAS§ that succeeds
only if the second address also matches its expected value.
§DCSS§ also provides the wait-free §DCSS\_READ§ primitive,
which can read the fields that can be concurrently modified by a §DCSS§.
Both are efficiently implemented using single-word
§CAS§es~\cite{Harris:2002:PMC:645959.676137,DBLP:conf/wdag/Arbel-Raviv017}.

%After a new node is inserted,
%we increment the §count§ fields of all ancestors to record the insertion.
%To reduce contention (especially near the root),
%we only perform these increments with some probability.
%Finally, we use the §count§ fields of all ancestors
%to compute an (over-)estimate
%of how imbalanced the subtrees rooted at these ancestors have become,
%and trigger subtree rebuilding if appropriate.
%
%One challenge in implementing insertion is synchronizing insertions
%with subtree rebuilding operations.
%In a naive implementation, if an insertion is performed
%in a subtree that is concurrently being rebuilt,
%then the insertion might be performed
%in a part of the subtree that is subsequently replaced.
%In this scenario, the insertion might appear to have succeeded
%(from the perspective of the invoking thread),
%even though it had no effect on the data structure.

%To avoid such problems,
%we require been been updates and subtree rebuilding operations
%to synchronize via the §status§ fields of nodes.
%Specifically, a subtree rebuilding operation can only rebuild a subtree
%after it ensures that every node in the subtree has a non-zero §status§ field.
%And, an insertion can only modify a node whose §status§ field is zero.

%This means whenever an insertion operation modifies a node,
%it must also atomically verify that the node's §status§ is zero.
%We accomplish such modifications
%using an atomic double-compare-single-swap (DCSS) primitive.
%This primitive takes two addresses,
%two expected values, and one new value as its arguments,
%and behaves like a CAS that succeeds
%only if the second address also matches its expected value.
%DCSS also provides another primitive called DCSS\_READ,
%which must be used to read any field that could be concurrently modified by a DCSS.
%DCSS can be implemented efficiently
%from single word CAS~\cite{DBLP:conf/wdag/Arbel-Raviv017}.

\begin{figure}[!t]
\begin{lstlisting}[firstnumber=1]
procedure insert(ist, key, val)
  path = [] °\hfill° // Stack that saves the path.
  n = ist.root
  while true
    index = interpolationSearch(key, n) °\label{lst:insert-interpolation-search}° °\ap{This was here -- should we remove it? -> affectsChangeSum = true}°
    child = DCSS_READ(n.children[index])
    if child is Inner
      n = child
      path.push( [child, index] )
    else if child is Empty | Single
      r = createFrom(child, key, val)
      result =
        DCSS(n.children[index], child, r, n.status, [0,°$\bot$°,°$\bot$°])°\label{lst:insert-dcss}°
      if result == FAILED_MAIN_ADDRESS
        continue °\hfill° // Retry from the same n.
      else if result == FAILED_AUX_ADDRESS
        return insert(ist, key, val) °\hfill°// Retry from the root.
      else
        for each [n, index] in path
          FETCH_AND_ADD(n.count, 1) °\label{lst:insert-fetch-and-add}°
        parent = ist.root
        for each [n, index] in path
          count = READ(n.count)
          if count >= REBUILD_THRESHOLD * n.initSize °\label{lst:insert-threshold}°
            rebuild(n, parent, index)
            break °\hfill°// exit for °\ap{Should we break as soon as you find the highest node for rebuild?}° °\ap{Can these 2 loops be fused into one? Seems like we can break as soon as we find a rebuild-point.}°
          parent = n
        return true
    else if child is Rebuild
      helpRebuild(child)
      return insert(ist, key, val) °\hfill° // Retry from the root.
\end{lstlisting}
\caption{Insert Operation}
\label{algo:insert}
\end{figure}

\paratitle{Insertion}
Figure~\ref{algo:insert} shows the pseudocode for §insert§,
which traverses the C-IST starting at the §root§.
An interpolation search \cite{Perl:1978:ISL:359545.359557}
is done at each node to determine the §index§ of the next child pointer for the given §key§.
This search uses the linear interpolation between the node's minimum
and maximum keys to estimate the index (in the node's array of keys)
to which the specified key belongs,
and does a linear search thereafter.
Since the §keys§ array does not change after the creation of an §Inner§ node,
§interpolationSearch§ has a sequential implementation, not shown here.
% \tb{note: ``linearly'' added}
% \ap{
% Is that still interpolation search? Or should another interpolation search ensue after a miss?
% }
% \ap{In the original IST, the same kind of search was used, apparently.}
%Then, starting from this estimated index,
%it linearly searches left or right as necessary to either find $key$,
%or find a pair of keys $k_i$ and $k_j$ such that $k_i < key < k_j$.
%The search returns an §index§
%of the next child pointer.
%This \textit{child} pointer is read using
%a special operation called DCSS\_READ, which is described below.

Next, §insert§ checks the type of the §child§ node.
If §child§ is an inner node, then §insert§ continues the traversal,
and at the same time adds the §child§ to the list called §path§.
This list is used to update the counts, as explained shortly.
%(This \textit{path} will be used after inserting a new node to revisit its ancestors.)
If §child§ is an §Empty§ or a §Single§ node,
then §insert§ replaces it with a new node §r§ with one or two keys, respectively,
allocated in the §createFrom§ subroutine.
%Let $v$ be a new §Single§ node that contains $key$.
%If $u$ is §Empty§, or $u$ is a §Single§ node that already contains $key$,
%then its \textit{r} is $v$.
%Otherwise, if $u$ is a §Single§ node that does not contain $key$,
%then its \textit{r} is a new §Inner§ node that points to $u$ and $v$.
%(The key of the internal node is the larger of \textit{key} and \textit{u.key}.)
The §DCSS§ in line \ref{lst:insert-dcss} inserts the new node
by changing §n.children[index]§ from §child§ to §r§
only if §n.status == [0,§$\bot$§,§$\bot$§]§.

The §DCSS§ in line \ref{lst:insert-dcss}
fails when §n.status $\neq$ [0,§$\bot$§,§$\bot$§]§,
and returns the §FAILED\_AUX\_ADDRESS§ value,
which indicates that the node is a part of an ongoing a rebuild.
In this case, §insert§ restarts from the root to find the §Rebuild§ node,
and help complete the rebuild.
The §DCSS§ could also fail if §n.children[index] $\neq$ child§,
indicating that another §insert§ or §delete§ or §rebuilding§ operation
modified the same location.
In this case, §insert§ restarts from the same §n§.
\tb{added rebuilding operation, because a pointer could be changed by a completed rebuilding operation...}
\ap{Agreed.}
%In the former case, the node is part of a subtree rebuild operation,
%and it may even have been removed from the tree already.
%%So, if the insertion \textit{were} performed,
%%the newly inserted nodes might be lost when the subtree is rebuilt.
%So, the \textit{insert} restarts at the root.
%Intuitively, after it restarts,
%it will either see that the subtree rebuild operation has already finished,
%or it will \textit{help} the subtree rebuild operation to complete.
%We further explain how this helping works, and why this guarantees progress, below.
%In the latter case, the node was concurrently modified by another \textit{insert}
%or \textit{delete} operation,
%and it may still be possible for this \textit{insert} operation
%to continue starting from $u$.
%(Note that $u$ can only be removed from the tree by a subtree rebuilding operation,
%and only after changing \textit{u.status} to a non-zero value,
%so we will never modify a deleted node.)
If the §DCSS§ is successful,
then §insert§ increments the §count§ fields
with the §FETCH\_AND\_ADD§ in line \ref{lst:insert-fetch-and-add}.
\tb{maybe get rid of sampling}
\ap{I removed it.}
\ap{
How did we pick 1/4? Did we experiment with other values?
Showing insert/lookup performance curves for different values might be interesting.
}

%(Note that some of these nodes might already have been replaced
%by a concurrent subtree rebuild operation $O$.
%It is not a problem that we increment the counts of these replaced nodes,
%instead of the nodes that replaced them,
%since the §count§ field stores the number of changes that occur in a subtree
%since it was last rebuilt, and our insertion must have occurred \textit{before}
%the subtree was rebuilt.
%(Otherwise, our insertion would have failed,
%since its DCSS will not modify a deleted node.))
%\trevor{Should we explain somewhere why these nodes
%(which may have been replaced by rebuilding) are still the ones we want to increment?
%}

Finally, the §insert§ searches the ancestors in §path§
for the highest node whose §count§ reached the threshold.
The threshold is checked in line \ref{lst:insert-threshold},
where §REBUILD\_THRESHOLD§ is set to $0.25$
(explained in Section 4 of the corresponding tech report~\cite{techreport-2020-c-ist}).
\tb{maybe get rid of sampling}
\ap{I removed the mention of $\epsilon$ and $q$.}
If such a node exists,
then §insert§ calls §rebuild§ to recreate the respective subtree.
As explained in Section~\ref{sec:partial-rebuild},
§rebuild§ inserts a §Rebuild§ node into the IST.
When other updates see this node,
they help complete the rebuild before proceeding.
%A §Rebuild§ object is essentially a node with a single child pointer
%that is inserted between a parent and a child
%to indicate that the subtree rooted at the child will be rebuilt.
%It also functions as a special \textit{descriptor} that specifies
%how other threads can help the subtree rebuild operation to complete.
%Whenever \textit{insert} encounters such an object,
%it first invokes a procedure called \textit{helpRebuild}
%to \textit{help} the rebuild operation complete, and then
%%continues as usual.
%restarts its traversal from the root.
%%\trevor{
%Is it necessary to restart from the root?
%It seems like we could restart from \textit{node}.
%}

% I realized that a tail-recursive loop solution might not be feasible,
% even with the lazy propagations.
% The reason is that our best target calculation was incorrect
% (i.e. it was greedily taking lower nodes just because they overflowed more).
%
%\begin{algorithm}[]
%\caption{Insert Operation}
%\label{algo:insert}
%\small
%\Proc{insert(ist, key)}{
%  node = ist.root\;
%  target, minLeft, minParent, minIndex = $\bot$, $\infty$, $\bot$, -1\;
%  path = [$\,$]\;
%  \While{true}{
%    index = interpolationSearch(node, key)\;
%    child, status = DCSS\_READ(node.children[index])\;
%    \If{status $\neq$ SUCCESS}{
%      \Return insert(ist, key)\;
%    }
%    \Switch{type(child)}{
%      \Case{Inner:}{
%        left = $\frac{1}{4} \cdot q \cdot$ child.initSize -
%          child.count + 1\;
%        \If{target = $\bot$ $\vee$ left < minLeft}{
%          target, minLeft, minParent, minIndex = child, left, node, index\;
%        }
%        node = child\;
%        path = path $\concat$ [child]\;
%      }
%      \Case{Empty | Single:}{
%        r = createFrom(child, key)\;
%        status = DCSS(node.children[index], child, r, node.status, 0)\;
%        \uIf{status = FAILED\_MAIN\_ADDRESS}{
%          \textit{// Retry from the same node.}
%        }
%        \uElseIf{status = FAILED\_AUX\_ADDRESS}{
%          \Return insert(ist, key)\;
%        }
%        \Else{
%          \If{random() < $q$}{
%            \For{node $\leftarrow$ path}{
%              FETCH\_AND\_ADD(node.count, 1)\;
%            }
%          }
%% ----------------
%% This is the initial lazy version:
%%          FETCH\_AND\_ADD(node.count, 1)\;
%% ----------------
%          \If{target $\neq$ $\bot$ $\wedge$ remaining <= 0}{
%            rebuild(target, parent, index)\;
%          }
%          \Return true\;
%        }
%      }
%      \Case{Rebuild:}{
%        helpRebuild(child)\;
%        \Return insert(ist, key)\;
%      }
%    }
%  }
%}
%\end{algorithm}

\paratitle{Deletion}
The §delete§ either replaces a §Single§ node with a new §Empty§ node,
or does not change the data structure if the key is not present.
It is almost identical to §insert§ --
the main difference is that when §child§ is an §Empty§ node,
§delete§ simply returns §false§,
and when §child§ is a §Single§,
instead of calling §createFrom§,
the node is replaced an §Empty§ if the keys match.
The deletion does not shrink §Inner§ nodes --
while some §Empty§ nodes can accumulate in the tree,
then the rebuilding operations eventually remove them.
With our chosen threshold, at most $25\%$ of all nodes can be §Empty§.
% \tb{measure how many}


\subsection{Partial Rebuilding}
\label{sec:partial-rebuild}

When insertion or deletion detects that a subtree rooted at a node $target$
(henceforth, the ``target subtree'') has become sufficiently imbalanced,
it rebuilds the subtree, as shown in Figure \ref{algo:rebuild}.
Rebuilding has four steps.
First, a thread announces the intention by creating a §Rebuild§ descriptor,
and inserts the descriptor between the $target$ and its $parent$.
Second, the thread does a preorder traversal of the subtree,
and sets a bit in the §status§ field of each node to prevent further updates.
Third, the thread creates an ideal IST (rooted at $ideal$)
using the old subtree's keys (rooted at $target$).
Finally, the old subtree is replaced with the new subtree in the parent.

\begin{figure}[!ht]
\begin{lstlisting}
procedure rebuild(node, p, i)
  op = new Rebuild(node, p, i)
  result = DCSS(p.children[i], node, op, p.status, [0,°$\bot$°,°$\bot$°]) °\label{lst:rebuild-dcss}°
  if result == SUCCESS then helpRebuild(op)

procedure helpRebuild(op)
  keyCount = markAndCount(op.target) °\label{lst:help-rebuild-mark}°
  ideal = createIdeal(op.target, keyCount) °\label{lst:help-rebuild-create-ideal}°
  p = op.parent
  DCSS(p.children[op.index], op, ideal, p.status, [0,°$\bot$°,°$\bot$°])°\label{lst:help-rebuild-dcss}°

procedure markAndCount(node) °\label{lst:mark-declaration}°
  if node is Empty then return 0
  if node is Single then return 1
  if node is Rebuild then return markAndCount(op.target)
  // node is Inner
  CAS(node.status, [0,°$\bot$°,°$\bot$°], [0,°$\bot$°,°$\top$°]) °\label{lst:mark-cas-0-1}° °\label{lst:mark-end-of-preamble}°
  keyCount = 0 °\label{lst:mark-start-of-postamble}°
  for index in 0 until length(node.children) °\label{lst:mark-loop}°
    child = READ(node.children[index])
    if child is Inner then
      [count, finished, started] = READ(child.status)
      if finished then keyCount += count
      else keyCount += markAndCount(child) °\label{lst:mark-end-loop}°
    else if child is Single then keyCount += 1
  CAS(node.status, [0,°$\bot$°,°$\top$°], [keyCount,°$\top$°,°$\top$°]) °\label{lst:mark-cas-1-keycount}°
  return keyCount °\label{lst:mark-end}°
\end{lstlisting}
\caption{Rebuild Operation}
\label{algo:rebuild}
\end{figure}

\paratitle{Implementation}
In the first step,
the §rebuild§ procedure creates the §Rebuild§ descriptor object,
and announces it with the §DCSS§ in line \ref{lst:rebuild-dcss}.
If this §DCSS§ is not successful,
then either there is another rebuild in some ancestor,
or another thread concurrently started the rebuild at the same node --
in both cases, the current thread can abort the rebuild.

If the announcement is successful,
rebuilding continues in the §helpRebuild§ subroutine.
If other threads need to update the respective subtree,
then they observe the §Rebuild§ node,
and help by also calling §helpRebuild§.
The call to §markAndCount§ traverses the subtree,
and sets the §status§ field of each inner node to $[0, \bot, \top]$
with the §CAS§ in line \ref{lst:mark-cas-0-1}.
At the same time,
§markAndCount§ counts the number of keys below each node,
and, once all the children are traversed,
it stores the total key count in the higher bits of the §status§ field
in line \ref{lst:mark-cas-1-keycount}.
The count allows computing the node degrees in the new subtree.
Note that, since the threads compete to set the same value in §status§,
the success of these two §CAS§es does not need to be checked --
exactly one thread succeeds.

The §createIdeal§ creates an ideal IST,
as defined in Section \ref{sec:data-types},
and ensures that the degree of each node is $\approx \sqrt{N}$,
where $N$ is the number of keys in that node's subtree.
We do not show its pseudocode,
since it involves no concurrency.
% \tb{include for completeness' sake in an appendix?}
% \ap{
% Yes, it makes sense to include it in the appendix.
% }

In the last step,
the old subtree is replaced with the new one
%new subtree is swapped in place of the old one % back into the parent
by the §DCSS§ in line \ref{lst:help-rebuild-dcss}.
If this §DCSS§ fails,
then either another thread finished the rebuild,
or another rebuild started in some ancestor,
so no further action is necessary.


\section{Concurrent Interpolation Search Tree with Collaborative Rebuilding}
\label{sec:concurrent-collaborative-rebuild}

% \trevor{some glue}

The basic rebuilding procedure, described in Section \ref{sec:insertion-deletion},
suffers from a scalability bottleneck when a lot of threads concurrently modify the IST.
Since multiple threads compete to mark the old subtree in the §markAndCount§ procedure,
and multiple threads create the same new subtree
in the §createIdeal§ procedure from Figure \ref{fig:concurrent-rebuild},
part of the work can be duplicated due to contention.
To address this, we designed and implemented a collaborative rebuilding algorithm,
in which threads mark and rebuild the subtree in parallel.


% \subsection{Data Types}

\begin{figure}[t]
% \begin{minipage}[t]{0.22\textwidth}
% \begin{lstlisting}[numbers=none]
% struct IST is
%   root: Node

% struct Single: Node is
%   key: KeyType
%   val: ValType
% \end{lstlisting}
% \end{minipage}
\begin{minipage}[t]{0.22\textwidth}
\begin{lstlisting}[numbers=none]
struct Rebuild: Node is
  target: Inner
  newTarget: Inner
  parent: Inner
  index: int
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.25\textwidth}
\begin{lstlisting}[numbers=none]
struct Inner: Node is
  initSize: int
  degree: int
  keys: KeyType[]
  children: Node[]
  status: [int, bool, bool]
  count: int
  nextMark: int
\end{lstlisting}
\end{minipage}
%\vspace{-4mm}
\caption{Modified Data Types for Collaborative Rebuilding}
\label{algo:data-types-cr}
\end{figure}


\subsection{Fast Collaborative Rebuilding}
\label{sec:concurrent-rebuild}

To enable threads to perform rebuilding \textit{collaboratively},
we make several changes in the algorithm. 
First, we replace the §markAndCount§ procedure with
a new procedure called §markAndCountCollaborative§,
in which helpers attempt to process different parts of the data structure
in parallel, and carefully avoid duplicating the work.

Second, we replace the call to §createIdeal§
% and the lines~\ref{lst:help-rebuild-create-ideal}-\ref{lst:help-rebuild-dcss}
inside the procedure §helpRebuild§
in Figure~\ref{algo:rebuild}
with a call to a new procedure §createIdealCollaborative§,
in which a new root of the subtree is first created
(which initially contains only §null§-pointers)
and \textit{announced}.
For this purpose, we add the §newTarget§ field to the §Rebuild§ data type,
as shown in Figure \ref{algo:data-types-cr},
to store the root node of the new subtree.
Each §null§-pointer in the new root of the subtree represents a ``job''
that a thread can perform by building the corresponding subtree
(and changing the §null§-pointer to point to this new subtree).
Of course, many of these jobs can be performed in parallel.
This way, until the new ideal IST is complete,
the §newTarget§ node serves as a sort of lock-free work queue.
Finally, we add the §nextMark§ field to §Inner§ nodes,
which is used in collaborative marking.

These subtlety of these changes is to distribute work
among threads while preserving lock-freedom,
which mandates that all work is done eventually,
even if some threads block.
% (hence, the conventional blocking approach of having threads
% exclusively reserve jobs to perform cannot be used here).
% \ap{Remark about blocking might be argued by reviewers, maybe remove?}

The collaborative rebuilding algorithm is illustrated in Figure~\ref{fig:concurrent-rebuild},
which we explain in the following paragraphs.

%\textbf{rebuild:}
%
%we first create a rebuild operation descriptor
%it points to the root of the subtree to be rebuilt: the "target"
%dcss is used to insert the rebuild op as a parent of the target
%if it fails, the descriptor is freed
%else helpRebuild is called
%
%\textbf{helpRebuild:}

\edef\lstMarkDeclaration{\getrefnumber{lst:mark-declaration}}
\edef\lstMarkEndOfPreamble{\getrefnumber{lst:mark-end-of-preamble}}
\edef\lstMarkStartOfPostamble{\getrefnumber{lst:mark-start-of-postamble}}

\begin{figure}[!t]
\begin{lstlisting}[
  firstnumber=\lstMarkDeclaration
]
procedure markAndCountCollaborative(node) °\Suppressnumber°
  // ... same as markAndCount until line °\textit{\ref{lst:mark-end-of-preamble}}°, but with
  // recursive calls to markAndCountCollaborative ... °\Reactivatenumber{\lstMarkEndOfPreamble + 1}°
  if node.degree > COLLABORATION_THRESHOLD °\label{lst:mark-cr-threshold}°
    while true °\label{lst:mark-cr-loop}°
      index = FETCH_AND_ADD(node.nextMark, 1)
      if index >= node.degree then break
      markAndCountCollaborative(node.children[index]) °\Suppressnumber° °\label{lst:mark-cr-end-loop}°
  // ... same as markAndCount from line °\textit{\ref{lst:mark-start-of-postamble}}°, but with
  // recursive calls to markAndCountCollaborative ...
\end{lstlisting}
\caption{The \texttt{markAndCountCollaborative} Procedure}
\label{algo:mark-and-count-collaborative}
\end{figure}

\paratitle{Collaborative marking algorithm}
Similar to the basic algorithm from Section~\ref{sec:algorithm},
the collaborative rebuilding algorithm starts by setting the §status§ field
of all the nodes in the subtree that must be rebuilt.
The main difference in the collaborative marking algorithm
is that it allows the helping threads to mark parts of the subtree in parallel.
The §markAndCountCollaborative§ procedure,
shown in Fig.~\ref{algo:mark-and-count-collaborative},
starts by setting the low boolean of the §status§ field,
and is the same as the basic §markAndCount§ from Fig.~\ref{algo:rebuild}
until line~\ref{lst:mark-end-of-preamble}.
If the number of children of the node is larger
than the §COLLABORATION\_THRESHOLD§ value (experimentally set to $48$),
the marking repetitively invokes the atomic §FETCH\_AND\_ADD§ instruction
on the §nextMark§ field, to get the index of the next free child
that can be recursively marked (line~\ref{lst:mark-cr-threshold}).
This allows multiple threads to concurrently mark the distinct children,
which reduces the memory contention.

The rest of the §markAndCountCollaborative§ procedure is exactly the same
as the §markAndCount§ procedure from Fig.~\ref{algo:rebuild}
after line~\ref{lst:mark-start-of-postamble}.
In particular, after executing the loop
in lines~\ref{lst:mark-cr-loop}-\ref{lst:mark-cr-end-loop}
of Fig.~\ref{algo:mark-and-count-collaborative},
collaborative marking does another pass through the node's §children§ array
to help the other threads that are slow.
In this second pass
(lines~\ref{lst:mark-loop}-\ref{lst:mark-end-loop} of Fig.~\ref{algo:rebuild}),
the thread recursively marks those children whose key-count was not yet computed.
This second pass is necessary to preserve lock-freedom --
if any of the other threads halts, the marking will complete in a finite number of steps.

\ap{
Trevor, could you please change 1-7 in the figure with the rebuilding to A-G?
I could not install latest 7.2.12 IPE on Ubuntu due to libjpeg62-turbo,
and after opening it in Wine, it seems that rebuild2.ipe is not the right version.
}

\paratitle{Collaborative marking example}
The collaborative marking is illustrated in Fig.~\ref{fig:concurrent-rebuild}.
The §Rebuild§ object is first announced in Fig.~\ref{fig:concurrent-rebuild}A.
At this point, the §status§ fields of all the inner nodes in the §target§ subtree
are set to §[0,§$\bot$§,§$\bot$§]§ (shown in the rightmost box of each node),
indicating that the marking has not started in any of those nodes.
In Fig.~\ref{fig:concurrent-rebuild}B, thread $p$ executed §FETCH\_AND\_ADD§
and decided to mark the child at index §0§,
while threads $q$ and $r$ are marking children at indices §1§ and §3§, respectively.
Thread $q$ has completed the marking
(indicated by the §[2,§$\top$§,§$\top$§]§ in the §status§ field of the corresponding child),
and can now help threads $p$ and $r$ to complete the marking
and set the key counts of their children.
In Fig.~\ref{fig:concurrent-rebuild}C, all the threads have finished marking,
and the §target§ node has the §status§ field set to §[9,§$\top$§,§$\top$§]§.
At this point, no more concurrent modifications of the §target§ subtree are possible,
and §target§ can be traversed without synchronization
for the purposes of creating a new subtree.

\edef\lstMarkEnd{\getrefnumber{lst:mark-end}}
\Reactivatenumber{\lstMarkEnd + 2}

\begin{figure}[!ht]
\begin{lstlisting}[
]
procedure createIdealCollaborative(op, keyCount)
  if keyCount < COLLABORATION_THRESHOLD then
    newTarget = createIdeal(op.target, keyCount) °\label{lst:create-ideal-cr-sequential}°
  else
    newTarget = new Inner( °\label{lst:create-ideal-cr-new-inner}°
      initSize = keyCount,
      degree = 0, // Will be set to final value in line °\textit{\ref{lst:create-ideal-cr-cas-degree}}°.
      keys = new KeyType[°$\lfloor\sqrt{\texttt{keyCount}}\rfloor$° - 1],
      children = new Node[°$\lfloor\sqrt{\texttt{keyCount}}\rfloor$°],
      status = [0, °$\bot$°, °$\bot$°], count = 0, nextMark = 0)
  if not CAS(op.newTarget, null, newTarget) then °\label{lst:create-ideal-cr-cas-new-target}°
    // Subtree root was inserted by another thread.
    newTarget = READ(op.newTarget) °\label{lst:create-ideal-cr-read-new-target}°
  if keyCount < COLLABORATION_THRESHOLD then
    while true °\label{lst:create-ideal-cr-loop}°
      index = READ(newTarget.degree)
      if index == length(newTarget.children) then break
      if CAS(newTarget.degree, index, index + 1) then °\label{lst:create-ideal-cr-cas-degree}°
        if not rebuildAndSetChild(op, keyCount, index)
          return newTarget °\label{lst:create-ideal-cr-end-loop}°
    for index in 0 until length(newTarget.children) °\label{lst:create-ideal-cr-for-loop}°
      child = READ(newTarget.children[index])
      if child == null then
        if not rebuildAndSetChild(op, keyCount, index)
          return newTarget °\label{lst:create-ideal-cr-end-for-loop}°
  return newTarget

procedure rebuildAndSetChild(op, keyCount, index)
  // Calculate the key interval for this child, and rebuild.
  totalChildren = °$\lfloor\sqrt{\texttt{keyCount}}\rfloor$°
  childSize = °$\lfloor$°keyCount / totalChildren°$\rfloor$°
  remainder = keyCount % totalChildren
  fromKey = childSize * index + min(index, remainder)
  childKeyCount = childSize + (index < remainder ? 1 : 0)
  child = createIdeal(op.target, fromKey, childKeyCount) °\label{lst:rebuild-and-set-create-ideal}°
  if index < length(op.newTarget.keys)
    key = findKeyAtIndex(op.target, fromKey)
    WRITE(op.newTarget.keys[index], key) °\label{lst:rebuild-and-set-write-key}°
  // Set new child, check if failed due to status change.
  result = DCSS(op.newTarget.children[index], °\label{lst:rebuild-and-set-dcss}°
    null, child, op.newTarget.status, [0, °$\bot$°, °$\bot$°])
  return result != FAILED_AUX_ADDRESS
\end{lstlisting}
\caption{The \texttt{createIdealCollaborative} Procedure}
\label{algo:create-ideal-cr}
\end{figure}

\begin{figure*}[t]
  \includegraphics[width=0.94\textwidth]{figures/rebuild3.pdf}
  \caption{Illustration of the collaborative rebuilding algorithm.}
  \label{fig:concurrent-rebuild}
\end{figure*}

\paratitle{Collaborative building}
After the §target§ subtree is marked, and the total key-count is known,
the algorithm allocates the root node of the new subtree.
Once again, if the key-count is below the §COLLABORATION\_THRESHOLD§,
the entire subtree is created without collaboration
with the call to the §createIdeal§ procedure,
in line~\ref{lst:create-ideal-cr-sequential}
of Fig.~\ref{algo:create-ideal-cr}.
If the key-count is above this level,
a new root node is allocated in line~\ref{lst:create-ideal-cr-new-inner}.
The size of the children array is set to the square root of the key-count.
Notably, the §degree§ field is initially set to §0§,
but it is later used in line~\ref{lst:create-ideal-cr-cas-degree}
to enable threads to coordinate between the child slots that they work on,
and is set to the proper value by the time the rebuilding completes.

Once the root node of the new subtree is allocated,
threads compete to write it into the §newTarget§ field of the §Rebuild§ object,
in line~\ref{lst:create-ideal-cr-cas-new-target}.
After the new root is announced,
threads atomically increment the §degree§ field to select a child index to work on,
in lines~\ref{lst:create-ideal-cr-loop}-\ref{lst:create-ideal-cr-end-loop}.
Upon acquiring an index, a thread calls the §rebuildAndSetChild§ procedure.
This procedure calculates the interval of keys from the original subtree for the new child,
and then calls §createIdeal§ to create the child tree.
The §createIdeal§ procedure is not shown due to space reasons,
but it is a straightforward traversal of the original tree --
since the original is effectively immutable, no synchronization is necessary.
After the new child is created,
the thread runs a §DCSS§ in line~\ref{lst:rebuild-and-set-dcss}
to write the child into the array.
If §DCSS§ fails due to a change in the §status§ field,
then this means that another rebuild operation is ocurring higher in the tree.
In this case, §rebuildAndSetChild§ returns §false§ to the caller,
allowing it to stop rebuilding early.
Notably, the key is written non-conditionally into the §keys§ array
in line~\ref{lst:rebuild-and-set-write-key},
since potential helpers write the same value.

When the §degree§ gets equal to the length of the §children§ array,
it means that some thread had started creating a new child at every entry of the array
(moreover, some threads could have already created a new child,
and set an entry in the §children§ array to point to that new child).
To guarantee lock-freedom, if a thread cannot increment §degree§ further,
then it must help the slow threads complete their own children.
In lines~\ref{lst:create-ideal-cr-for-loop}-\ref{lst:create-ideal-cr-end-for-loop},
a thread checks the entries of the §children§ array,
and helps rebuild the children at entries whose value is still §null§.
The rebuilding is completed once all the entries are non-§null§.

\paratitle{Collaborative building example}
The collaborative subtree rebuilding is illustrated in Fig.~\ref{fig:concurrent-rebuild}D-G.
After the §target§ subtree is marked, and is determined to have $9$ keys in total,
the threads compete to announce the root of the new subtree
with a §DCSS§ instruction in Fig.~\ref{fig:concurrent-rebuild}D.
The newly announced node has $\sqrt{9}=3$ entries,
so each of its children will cover $9/\sqrt{9}=3$ keys.
In Fig.~\ref{fig:concurrent-rebuild}E,
thread $p$ acquired the index $0$ of the §children§ array,
and determined that it needs to collect
the keys $k_1$, $k_2$ and $k_3$ of the original subtree (shown in gray).
Thread $p$ allocated a new child node of size $3$,
and used §DCSS§ to enter that child into the §children§ array.
In Fig.~\ref{fig:concurrent-rebuild}F,
another thread had built and stored the child at index $2$ of the §children§ array,
while the thread $q$ is the only thread that is still working on the index $1$.
Helping threads can now enter
the lines~\ref{lst:create-ideal-cr-for-loop}-\ref{lst:create-ideal-cr-end-for-loop}
of the pseudocode in Fig. \ref{algo:create-ideal-cr},
and can compete with the thread $q$ to populate the index $1$.
In Fig.~\ref{fig:concurrent-rebuild}G,
the rebuilding is completed, and the threads compete to replace the §Rebuild§ object
with the new, ideal subtree.

% \ap{
% Any idea how often, quantitatively, a rebuild is preempted by a rebuild higher in the tree?
% }

% \ap{
% Any idea on which percentage of time is spent by stragglers when completing a rebuild?
% }

% \ap{
% Any idea on how much helping actually helps in terms of performance?
% If it does considerably, then would some coordinated, rather than random,
% offset-selection be much better (in createIdealCollaborative)?
% One question might be why did we pick a random offset.
% }

\ap{
Can we plot a graph that shows the relationship between performance,
and the value of COLLABORATIVE\_THRESHOLD?
}


\subsection{Lookups and Range Queries}
%\subsection{Lookups, Predecessor and Range Queries}
\label{sec:lookups-and-queries}

The §lookup§ subroutine, shown in Figure~\ref{algo:lookup},
is similar to the §insert§.
An interpolation search is repeated until reaching an §Empty§ or a §Single§ node.
If it reaches a §Single§ node that contains the specified key,
it returns §true§.
Otherwise, if §lookup§ encounters an §Empty§ node or
a §Single§ node that does \emph{not} contain the specified key,
it returns §false§.
%If it reaches an §Empty§ node, then $key$ is not in the data structure,
%so \textit{lookup} returns false.
%Similarly, \textit{lookup} returns false if it reaches
%a §Single§ node that does \textit{not} contain $key$.
%If it reaches a §Single§ node that contains key, it returns true.

If §lookup§ encounters a §Rebuild§ object,
it simply follows the §target§ pointer
to move to the next node, and continues traversal.
Unlike the §insert§ operation,
§lookup§ does not help concurrent subtree rebuilding operations.
Lookups do not need to help rebuilding to ensure progress,
and so they avoid the unnecessary overhead.
%This would contradict our design goals.
%Note that \textit{lookup} never needs to restart from the root.
Apart from its use of DCSS\_READ and the handling of §Rebuild§ objects,
\textit{lookup} is effectively a sequential interpolation tree search.

%\paragraph*{Predecessor queries}
%
%Note that \textit{lookup} can be extended to provide non-blocking \textit{predecessor}$(ist, key)$ queries.
%The idea is to modify \textit{lookup}$(ist, key)$ to remember the lowest common ancestor $u$ of $key$ and its predecessor.
%In a binary search tree, the lowest common ancestor is the last node where the \textit{lookup} followed the \textit{right} child pointer.
%In the IST, the lowest common ancestor is the last node where the \textit{lookup} followed a pointer $\textit{u.children}[\textit{index}]$ where $\textit{index} > 0$ (i.e., \textit{not} the leftmost pointer).
%
%So, \textit{predecessor}$(ist, key)$ traverses the tree looking for $key$, and remembers the lowest common ancestor $u$ of $key$ and its predecessor.
%Once \textit{predecessor} reaches an §Empty§ or §Single§ node $v$, it returns to the lowest common ancestor $u$, follows the pointer just to the left (i.e., \textit{u.children}[$\textit{index}-1$]), and then performs a depth-first search (DFS) starting from \textit{u.children}[$\textit{index}-1$] that traverses pointers from right to left (i.e., traversing the rightmost pointer first).
%This DFS terminates when it encounters a §Single§ node $w$, or when it discovers that all .......................... \trevor{problem: might need to DFS the entire tree}.
%%the rightmost child pointer it sees until it reaches an §Empty§ or §Single§ node $w$.
%%If $w$ is 
%
%Finally, we must ensure that there is a time during the \textit{predecessor} when $w$ is in the IST and $w.key$ is the predecessor of $key$.
%The easiest way to do this is simply to repeat the steps taken so far, and check whether the \textit{predecessor} reaches the same nodes $v$ and $w$ again.
%If so, we are done.
%If not, the \textit{predecessor} operation simply restarts (which preserves non-blocking progress, because a concurrent update operation completed).
%
%%Since the IST stores several keys in each
%%most of the time, pred/succ will be in the same node? (only if we get rid of separate leaf nodes and embed several keys/values directly in fat leaf nodes.)

\paratitle{Range queries}
In some applications it is useful to have access to
non-blocking \textit{range query} operations,
which return all of the keys in the data structure
that intersect some range $[low, high]$.
The IST could be augmented with support for range query operations using,
for example, the recently introduced methodology of
Arbel-Raviv and Brown~\cite{Arbel-Raviv:2018:HER:3178487.3178489}.

\begin{figure}[!t]
\begin{lstlisting}
procedure lookup(ist, key)
  n = ist.root
  while true
    if n is Inner then
      index = interpolationSearch(key, n)
      n = DCSS_READ(n.children[index]) °\label{lst:lookup-dcss-read}°
    else if n is Single then return n.k == key ? n.v : null
    else if n is Empty then return null
    else if n is Rebuild then n = n.target
\end{lstlisting}
\caption{Lookup Operation}
\label{algo:lookup}
\end{figure}

% \paratitle{Memory reclamation}

% \tb{todo: describe memoyr reclamation using epoch based reclamation...}
% \ap{commented out for now}



==> parts/analysis.tex <==
% !TEX root = ../main.tex

\begin{figure*}[!ht]
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_0p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_0p_k_2x10_7.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_0p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_0p_k_2x10_9.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_1p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_1p_k_2x10_7.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_1p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_1p_k_2x10_9.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_10p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_10p_k_2x10_7.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_10p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_10p_k_2x10_9.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_40p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_40p_k_2x10_7.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_40p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/throughput/exp1_scaling_threads_throughput_exp_u_40p_k_2x10_9.png}

% \includegraphics[scale=0.25]{experiments/throughput/exp1_scaling_threads_throughput_legend.png}
\caption{
Basic Operations Throughput, Higher is Better
(\crule[Gray]{2mm}{2mm} NM,
\crule[Bluish]{2mm}{2mm} BCCO,
\crule[BloodOrange]{2mm}{2mm} ABTree,
\crule[SunsetYellow]{2mm}{2mm} ISTree)
}
\label{fig:evaluation:basic-operations}
\end{figure*}

\section{Analysis}
\label{sec:analysis}

This section contains an outline of the correctness proofs and the complexity analysis
of the C-IST data structure.
For reasons of space, we only list the most important lemmas and theorems,
and keep the rest in the appendix.


\subsection{Safety, Linearizability and Lock-Freedom}

To prove correctness, we associate the C-IST and its operations
with the semantics of an abstract set $\mathbb{A}$.

\begin{definition}[Consistency]
  An C-IST §I§ is \emph{consistent} with an abstract set $\mathbb{A}$
  if and only if $\forall k \in \mathbb{A} \Leftrightarrow \haskey(§I§, k)$.
\end{definition}

By identifying the atomic instructions
at which the corresponding abstract set $\mathbb{A}$ changes,
we show that a C-IST operation changes the corresponding set exactly once.
At the same time, we identify instructions that change the state of the data structure,
but not the state of the corresponding abstract set.
The linearizability proof follows naturally.

% \begin{lemma}[Freezing]
%   \label{lem:freeze}
%   After §markAndCount§
%   in line \ref{lst:help-rebuild-mark} of Figure \ref{algo:rebuild} completes,
%   all the nodes in the corresponding subtree have a non-zero §status§.
% \end{lemma}

% \begin{lemma}[Cover stability]
%   \label{lem:cover-stability}
%   If a node §n§ covers the interval $[ a, b \rangle$ at some time $t_0$,
%   then §n§ covers the same interval $\forall t > t_0$,
%   as long as §n§ is reachable at the time $t$.
% \end{lemma}

\begin{theorem}[Safety]
  \label{thm:safety}
  An C-IST §I§ is always valid and consistent with some abstract set $\mathbb{A}$.
  C-IST operations are consistent with the operational semantics of the abstract sets.
\end{theorem}

\begin{corollary}[Linearizability]
  Lookup, insertion and deletion operations are linearizable.
\end{corollary}

To show lock-freedom of the modification operations,
we show that, for any C-IST,
only finitely many data structure changes occur
before the corresponding abstract set changes.

\begin{lemma}
There is a finite number of steps between any two C-IST modifications,
and there are finitely many consecutive modifications
that do not change the abstract set.
\end{lemma}

\begin{theorem}[Non-Blocking]
  \label{thm:non-blocking}
  Insertion and deletion are lock-free, and lookup is wait-free.
\end{theorem}


\subsection{Complexity}

The complexity analysis for C-IST follows the argument for sequential ISTs~\cite{IST},
with modifications due to the fact that
at any time there can be up to $p$ threads that are concurrently modifying the C-IST. 
The complete arguments can be found in the additional material. 
In particular, the worst-case depth bound is the following: 

\begin{lemma}
\label{lem:worst-case-depth}
Let $p$ be the number of concurrent threads that are modifying a C-IST.
Worst-case depth of a C-IST that contains $n$ keys is $O(p + \log n)$.
\end{lemma}


In turn, a standard amortization argument implies the following naive worst-case amortized bound:
\begin{lemma}
\label{lem:amortized-cost}
The worst-case amortized cost of insert and delete operations,
without including the cost of searching for the node in the C-IST,
is $O(\gamma (p + \log n))$, where $\gamma$ is a bound on the average interval contention.
\end{lemma}

The above worst-case bound can probably be further tightened. 
However, our main focus is on \emph{expected amortized} bounds,
which allow us to go below $\Theta(\log n)$.
The following holds for the expected amortized cost of updates:

\begin{lemma}
\label{lem:amortized-expected-log-log}
Let $\mu$ be a probability density with a finite support $[a, b]$.
The expected total cost of processing
a sequence of $n$ $\mu$-random insertions and uniformly random deletions
into an initially empty C-IST is $O(n(\log \log n + p) \gamma)$, 
where $\gamma$ is a bound on average interval contention. 
\end{lemma}

We note that, for worst-case schedules, the value of $\gamma$ can be $\Theta(p)$,
although in practice we expect it to be lower. 
For searches, the following holds: 

\begin{lemma}
Let $\mu$ be a smooth probability density,
as defined Mehlkorn and Tsakalidis~\cite{IST},
for a parameter $\alpha$, such that $\frac{1}{2} \leq \alpha < 1$.
The expected search time in a $\mu$-random IST of size $n$ is
$O(\log \log n + p )$. 
\end{lemma}






 

==> parts/collaborative-notes.tex <==
markAndCount starts at the target.
at each recursive step that visits a node "current:"
if current is a kvpair: we return count 1.
if current is an "empty" value: we return count 0.
if current is a non-empty value: we return count 1.
if current is a rebuildop: we recurse on the node it points to.
finally, if current is a node:

we first check if another helper has already finished markAndCount
on the subtree rooted at current, by inspecting its dirty field.
dirty fields consist of a "started" bit, a "finished" bit, and a "count" subfield.
if the finished bit is set, then markAndCount has already finished on the subtree,
and the count has been stored in the "count" subfield,
so this subfield can immediately be returned.
otherwise, we use CAS to set the "started" bit,
indicating that a thread (us) is currently performing markAndCount on this subtree.
(if the started bit has already been set by a helper, then this CAS can be skipped.)
next, the thread will recursively call markAndCount on *each* of the pointers of current,
from left to right.
finally, we sum the values returned by our recursive calls,
and use CAS to store this sum in the "count" subfield of current.dirty.
(if we fail this CAS, it is because another thread already
computed the same sum and performed the same CAS.
the reason the computed sum will be the same is
that it is always computed using data in dirty nodes,
and dirty nodes never have their keys, values or pointers changed.)

%[example figure showing marking and counting]

OPTIMIZATION 
  to make helping more efficient in the event that
  several helpers concurrent work on the same subtree,
  before a thread starts recursing on the pointers of current,
  it first performs a fetch\&add on a "nextMarkAndCount" field of the current node.
  if the value returned by this fetch\&add is smaller than
  the number of pointers in the current node,
  then our thread will first optimistically recurse on *that* pointer of the current node first.
  this will cause multiple concurrent helpers to optimistically spread out
  and recurse on distinct subtrees of current to improve parallelism,
  rather than colliding on the same subtrees and causing needless memory contention.
  (if the value is larger than the number of pointers,
  then the number of helpers that have worked on this node
  is larger than the number of pointers, so we skip this optimistic step.
  we also skip this optimistic step if current is a leaf,
  since there is not much work to distribute between threads,
  and there is a smaller chance of helpers working in the same (tiny) subtree,
  so the cost of performing fetch\&add outweighs any potential benefits.)
  (note that it is still necessary for a thread to recurse on
  *all* of the pointers of current to guarantee lock freedom,
  since otherwise a thread could "reserve" a subtree to work on, and crash.
  note, however, that in the time our thread spends recursing on its first pointer,
  other helpers can finish their markAndCount calls on many of the other pointers.
  in this case, our recursive calls on those pointers will be fast.
  for each such pointer, we will simply see that the finished bit is set,
  and immediately return the saved count.)
  note that this (~15 line) algorithm elegantly distributes contending helper threads
  wherever they bump into one another, at all levels of the tree (except at leaves).

%[example figure showing optimistic thread distribution -- one simple case where k threads start helping a node at the same time, and one complex case where k threads all start helping and then a few more threads start helping in an already-occupied subtree]


\paragraph{CreateIdealCollaborative}
% \textbf{2. create ideal tree concurrently}
now that the target subtree has been entirely marked as dirty, it can no longer be changed in
any way. this makes it relatively easy to rebuild it into an ideal istree and atomically replace
it.

one naive lock free algorithm for doing this is to have each thread that is prevented from
performing an operation on this subtree (because it is dirty) to simply rebuild the entire
subtree itself, and *compete* with any other threads that are doing the same thing by attempting
to replace the old dirty subtree with *its own* newly created ideal subtree.

%[example figures with an empty tree, a kvpair, a leaf and a full tree]

a more efficient solution is to have enlist all such threads to *collaboratively* rebuild the
subtree in parallel. helping will be coordinated through a newly root node. at a high level, we
will create a new root node, and all helping threads will look at the pointers of this root node
to decide where to help. null pointers represent a subtree that has not yet been completed.

%[example figure showing root creation, election, and work distribution]

a pointer to this new root will be stored in the RebuildOperation object, in a field called
newTarget. note that this root node can only be created once we know how many keys are in the
subtree being rebuilt, so it must be allocated and have its pointer CASed into this
RebuildOperation object *after* markAndCount has already been performed on the target subtree.
to ensure lock-free progress, helping threads *compete* to allocate a new root node and CAS its
pointer into the RebuildOperation object. if the number n of key/value pairs found by
markAndCount is small enough that would fit in a single leaf, then the thread simply allocates a
leaf and fills it with these key/value pairs, and CASes a pointer to *this* node into the
RebuildOperation's newTarget pointer. (in this case, the newTarget CAS will *finish* the
rebuilding process.) if n is too large to fit in a single leaf, then a new internal node is
allocated with sqrt(n) pointers, and the thread CASes this node into op.newTarget. any thread
that *fails* to CAS its new root object into op.newTarget will free its own object, and simply
use the newTarget pointer that was stored by another thread.

if there are too many keys to fit into a leaf, then the thread will begin rebuilding at each
pointer of the new root, one at a time, starting at a pseudorandom offset (to scatter helpers)
and moving left to right. for each such pointer, the thread checks if it is still null (meaning
it has not been rebuilt yet), and if so calls subtreeBuildAndReplace on it.

%[example figure showing construction of one subtree]

suppose the new root has p pointers, and the target subtree contains k keys. each
subtreeBuildAndReplace call on one of these pointers will build an ideal istree containing
ceil(k/p) or floor(k/p) keys. (the number of trees with ceil(k/p) keys will be k mod p. the
remaining p - (k mod p) subtrees will contain floor(k/p) keys.)

suppose we label the keys in the target subtree 0 to k-1. subtreeBuildAndReplace uses the index
ix of the given pointer and the known number of keys k to compute the interval of keys (in the
target subtree) that it should contain. this works out to [s, t] where s=ix*floor(k/p) + min(ix,
p - (k mod p)) and t=s+floor(k/p) + (ix < (k mod p) ? 1 : 0).

[next up describe sequential builder and CASing subtree in...] given the interval [s, t], we use
depth-first search (DFS) with pruning to explore all nodes in the target subtree that can
contain keys in [s, t]. in this DFS, we use the subtree key counts that are stored at each node
(in the node.dirty.count field) to decide which subtrees can be pruned. more specifically,
throughout the DFS, we maintain a variable called "skipped" that contains the total number of
keys in all subtrees that have been pruned. to decide whether a subtree rooted at a node u can
be pruned, we first check whether skipped + u.dirty.count is smaller than s. if so, every key in
the subtree falls to the left of [s, t], so we can prune the subtree. if not, our DFS will
explore the subtree. whenever we encounter a key, we save it in an array called "pairs."

after the DFS, we invoke buildIdeal(pairs), which (sequentially) builds an ideal interpolation
search tree T from the keys in pairs. finally, we use CAS to change the appropriate pointer of
newTarget from null to T. if this CAS fails, then another thread already rebuilt this subtree.
(so, we free our subtree and move onto rebuild a different subtree.) the newly created subtree
has $count = 0$ for all nodes, since it is ideally balanced.

when all pointers of the newTarget are non-null, rebuilding is finished.

note that threads can continue to perform searches in the target subtree while it is being
rebuilt. any updating threads that enter the target subtree and encounter either the rebuild
operation object or a dirty node will help the rebuilding operation to complete before
continuing with their own operations.

[[[optimization: cut long tailed helping down by continually incrementally checking if the
subtree you are trying to build has already been completely built. abort at any time if this
occurs. we do this.]]]

subtreeBuildAndReplace could be further optimized by weaving the DFS into the buildIdeal
procedure to avoid the explicit construction of the pairs array. this optimization was not done.

\textbf{3. use dcss to change a pointer in parent, replacing rebuildRoot with newTarget} if dcss
succeeds, we retire the entire target subtree \trevor{this retiring is done collaboratively(!!)
with an algorithm in which threads take exclusive(!) ownership of nodes before retiring them,
and things are generally retired bottom-up. exclusive ownership isn't a problem for
lock-freedom, because the only consequence of a crashed thread is that some nodes won't be freed
ever. this is typically acceptable (and probably impossible to avoid). crashed threads don't
block progress because we are talking about objects that are NOT part of the data structure
anymore. doing this retire work collaboratively is critical to achieving high performance, since
long delays caused by sequential retire work lead to long reclamation epochs, which lead to
massive limbo lists in epoch-based reclamation, which leads to worse locality and higher batch
reclamation costs (due to high burst pressure on the allocator, which causes big delays in
allocator free() calls, and damages the allocator's ability to defray the cost of ``real''
malloc/free calls (which map/zero/purge/unmap pages) with object pooling/caching, since massive
working set size means caches are essentially always overflowed and released in response to
batch frees, but all of that memory will need to be allocated again to satisfy the huge working
set size, rendering overflowing/purging useless). that's a mouthful...} else if dcss fails
because the parent is dirty, the rebuildRoot is part of a larger subtree that is being rebuilt,
so we restart our operation (which will encounter that rebuild operation object and help it,
unless that rebuild operation has been completed by then) else if we fail because the parent's
pointer changed, it has already been changed to rebuildRoot by another helper

[example figure showing how nested rebuild inside another rebuild isn't a problem... either the
inner rebuild gets done first, and then its nodes get marked, or the inner one is slow, and the
outer one marks the parent first, in which case the inner one essentially ended up helping the
outer one markAndCount.]

[mention step 2 could be made more efficient with full recursive helping, like markAndCount, not
just helping at the top level?]

[optimization: if values fit in a single word, then leaves can directly inline values (storing
them in the pointer fields) instead of pointing to single nodes. and, empty nodes can simply be
represented by a dummy value.]


==> parts/conclusion.tex <==
% !TEX root = ../main.tex

\section{Conclusion}
\label{sec:conclusion}

We presented C-IST, the first concurrent
implementation of a dynamic interpolation search tree.
C-IST is non-blocking and scalable,
and it preserves the desirable complexity properties of the original data structure
with high probability.
Experimental results in C++ suggest that
C-IST significantly improves upon the performance
of classic search data structures with similar semantics,
by up to $\approx3.5\times$,
and the current best-performing alternative by up to $50\%$.

These findings suggest that concurrent data structure designs can be improved
in non-trivial ways by exploiting input-specific techniques developed in the sequential case.
We see this as an interesting line of potential future work.

==> parts/evaluation.tex <==
% !TEX root = ../main.tex

\section{Evaluation}
\label{sec:evaluation}


\begin{figure*}[t]
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_0p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_0p_k_2x10_7.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_0p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_0p_k_2x10_9.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_1p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_1p_k_2x10_7.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_1p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_1p_k_2x10_9.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_10p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_10p_k_2x10_7.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_10p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_10p_k_2x10_9.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_40p_k_2x10_6.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_40p_k_2x10_7.png}
% \includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_40p_k_2x10_8.png}
\includegraphics[scale=0.165]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_exp_u_40p_k_2x10_9.png}

% \includegraphics[scale=0.25]{experiments/llc_misses/exp1_scaling_threads_LLC_misses_legend.png}
\caption{
Last-Level Cache-Misses, Lower is Better
(\crule[Gray]{2mm}{2mm} NM,
\crule[Bluish]{2mm}{2mm} BCCO,
\crule[BloodOrange]{2mm}{2mm} ABTree,
\crule[SunsetYellow]{2mm}{2mm} ISTree)
}
\label{fig:evaluation:llc}
\end{figure*}

We implemented the concurrent IST in C++,
and compared it against several state of the art concurrent data structures.
We ran the benchmarks on a NUMA system with four Intel Xeon Platinum 8160 3.7GHz CPUs,
each of which has 24 cores and 48 hardware threads.
Within each CPU, cores share a 33MB LLC,
and cores on different CPUs do not share any caches.
The system has 384GB of RAM, and runs Ubuntu Linux 18.04.1 LTS.
Our code was compiled with GCC 7.4.0-1, with the highest optimization level (\texttt{-O3}).
Threads were \textit{pinned} to cores such that
thread counts up to 48 ran on only one CPU,
thread counts up to 96 run on only two CPUs,
and so on.
We used the fast scalable allocator jemalloc 5.0.1-25.
When a memory page is allocated on our 4-CPU Xeon system,
it has an \textit{affinity} for a single CPU,
and other CPUs pay a penalty to access it.
We used the \texttt{numactl --interleave=all} option to ensure
that pages are evenly distributed across CPUs.

We compared our IST implementation (ISTree) to the leading non-blocking binary search tree (NM)
due to Natarajan and Mittal~\cite{Natarajan:2014}, Bronson's concurrent AVL
tree~\cite{bronsonavl} (BCCO), which is the leading blocking binary search tree, and a fast
non-blocking $(a,b)$-tree (ABTree) due to Brown (Ch.8 of \cite{BrownPhD}), which is a
concurrency-friendly variant of a B-tree. (\textit{We also compared with many other concurrent
search trees}, which are omitted here.
See Section 5 in the corresponding technical report~\cite{techreport-2020-c-ist}
for details.)

The goal of the evaluation section is to show
that the amortized $O(\log \log n)$ running time
induces performance improvements on datasets that are reasonably large.
We therefore evaluate the C-IST operations
against other comparable data structures in Section~\ref{sec:evaluation:basic-operations},
where we show, for 1 billion keys, improvements ranging from $15$-$50\%$
compared to the $(a,b)$-tree~\cite{BrownPhD} (the next best alternative),
depending on the ratio of updates and lookups.
To further characterize the performance,
we compare the average key depth and the impact on cache behavior
in Section \ref{sec:evaluation:average-depth-and-cache},
and we show a breakdown of the execution time
in Section \ref{sec:evaluation:time-breakdown}.
We conclude with a comparison of memory footprints
in Section~\ref{sec:evaluation:memory-footprint}.

\begin{figure*}[ht]
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_1p_k_2x10_6_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_1p_k_2x10_7_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_1p_k_2x10_8_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_1p_k_2x10_9_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_10p_k_2x10_6_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_10p_k_2x10_7_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_10p_k_2x10_8_sequential_time_breakdown_Chart_4.png}
\includegraphics[scale=0.21]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_10p_k_2x10_9_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_40p_k_2x10_6_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_40p_k_2x10_7_sequential_time_breakdown_Chart_4.png}
% \includegraphics[scale=0.20]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_40p_k_2x10_8_sequential_time_breakdown_Chart_4.png}
\includegraphics[scale=0.21]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_40p_k_2x10_9_sequential_time_breakdown_Chart_4.png}
\includegraphics[scale=0.21]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_10p_k_2x10_9_collaborative_time_breakdown_Chart_4.png}
\includegraphics[scale=0.21]{experiments/rebuilding_time_breakdown/exp6_rebuilding_time_time_breakdown_exp2_u_40p_k_2x10_9_collaborative_time_breakdown_Chart_4.png}

\caption{
    Execution Time Breakdown
    (\crule[DarkBluish]{2mm}{2mm}~creating,
    \crule[Greenish]{2mm}{2mm}~marking,
    \crule[Bluish]{2mm}{2mm}~useless helping,
    \crule[BloodOrange]{2mm}{2mm}~deallocation,
    \crule[SunsetYellow]{2mm}{2mm}~locating garbage,
    \crule[Gray]{2mm}{2mm}~other).
    Bars are annotated with $f$, the number of times the \textit{root} (entire tree) was rebuilt.
}
\label{fig:evaluation:time-breakdown}
\end{figure*}

\begin{figure}[ht]
\includegraphics[scale=0.24]{experiments/disable_collaborative_rebuild/exp4_disable_rebuild_helping_pivot__.png}
\caption{
Comparison of Rebuilding Implementations
% (\crule[Gray]{2mm}{2mm} non-collaborative,
% \crule[Bluish]{2mm}{2mm} collaborative)
}
\label{fig:evaluation:collaborative-throughput}
\end{figure}

\subsection{Comparison of the Basic Operations}
\label{sec:evaluation:basic-operations}

Figure~\ref{fig:evaluation:basic-operations}
shows the throughput of concurrent IST operations,
compared against other sorted set data structures,
for dataset sizes of $k = 2 \cdot 10^8$ and $k = 2 \cdot 10^9$ keys,
and for $u = 0\%$, $u = 1\%$, $u = 10\%$ and $u = 40\%$,
where $u$ is the ratio of update operations among all operations.
Plots for additional dataset sizes are shown
in Figure~10 of the corresponding technical report~\cite{techreport-2020-c-ist}.

In all cases, C-IST operations have much higher throughput than
Natarajan and Mittal's non-blocking binary search tree (NM),
and concurrent AVL trees due to Bronson (BCCO).
For update ratios $u = 0\%$ and $u = 1\%$, concurrent IST also has a higher throughput
compared to Brown's non-blocking $(a,b)$-tree.
The underlying cause for better throughput is a lower rate of LLC misses
due to IST's doubly-logarithmic depth.
For higher update ratios $u = 10\%$ and $u = 40\%$,
the cost of concurrent rebuilds starts to dominate the gains of doubly-logarithmic searches,
and ABTree has a better throughput for $k = 2 \cdot 10^8$ keys.
Above $k = 2 \cdot 10^9$ keys,
ISTree outperforms ABTree even for the update ratio of $u = 40\%$.


\subsection{Average Depth and Cache Behavior}
\label{sec:evaluation:average-depth-and-cache}

The main benefit of C-IST's expected-$O(\log \log n)$ depth
is that the key-search results in less cache misses
compared to other tree data structures.
The plot shown below compares the average number of pointer hops required to reach a key
(error bars show min/max values over all trials),
for dataset sizes from $2 \cdot 10^6$ to $2 \cdot 10^9$ keys.
While the average depth is $20$-$40$ for NM and BCCO,
the average ABTree depth is between $6$ and $10$,
and the average C-IST depth is below $5$.

\begin{wrapfigure}{l}{0.22\textwidth}
\vspace{-5mm}
\noindent\includegraphics[scale=0.17]{experiments/avg_key_depth/exp1_scaling_threads_avg_key_depth__.png}
\vspace{-10mm}
\end{wrapfigure}
The differences in average depths between these data structures
correlate with the average number of cache misses.
Figure~\ref{fig:evaluation:llc} compares the average number of last-level cache-misses
between the different data structures, for different update ratios $u$.
For the dataset size of $2 \cdot 10^9$ keys,
ISTree operations undergo $2\times$ less cache misses,
and slightly fewer cache misses than ABTree.
A detailed set of plots for different dataset sizes
is shown in Figure~11 of the corresponding technical report~\cite{techreport-2020-c-ist}.

% \ap{
% How do you explain the raise in cache misses for higher thread counts?
% More time spent helping?
% If so, why is there a difference for $u = 0\%$? Higher LLC pressure with more threads?
% }


\subsection{Breakdown of the Execution Time}
\label{sec:evaluation:time-breakdown}

A breakdown of the execution time is shown in Figure~\ref{fig:evaluation:time-breakdown},
which contains plots for non-collaborative and collaborative rebuilding,
update ratios $u = 10\%$ and $u = 40\%$, and the dataset size $2 \cdot 10^9$.
In the non-collaborative variant, and for higher thread counts,
the execution time is dominated by the useless helping operations.
Since the work performed by the helping threads is discarded,
this results in scalability issues as the update ratio $u$ grows.
In the collaborative variant, this problem does not occur,
and most of the rebuilding time is spent in creating new subtrees.
A more detailed set of plots is shown
in Figure~12
and Figure~13
of the corresponding technical report~\cite{techreport-2020-c-ist}.

% \ap{Confirm - other includes the lookup operations?}


\begin{figure}[t]
\includegraphics[scale=0.20]{experiments/static_tree_mem_usage/exp2_memory_static_pivot_exp_u_40p_k_2x10_6.png}
\includegraphics[scale=0.20]{experiments/static_tree_mem_usage/exp2_memory_static_pivot_exp_u_40p_k_2x10_7.png}
\includegraphics[scale=0.20]{experiments/static_tree_mem_usage/exp2_memory_static_pivot_exp_u_40p_k_2x10_8.png}
\includegraphics[scale=0.20]{experiments/static_tree_mem_usage/exp2_memory_static_pivot_exp_u_40p_k_2x10_9.png}
\caption{
Memory Footprint Comparison
}
\label{fig:evaluation:memory-footprint}
\end{figure}

\subsection{Memory Footprint}
\label{sec:evaluation:memory-footprint}

Due to using a lower number of nodes for the same dataset,
the average space overhead is lower for the C-IST than the other data structures.
Figure~\ref{fig:evaluation:memory-footprint} shows
the different memory footprints for four different dataset sizes.
C-IST has a relative space overhead of $\approx$$30$-$100\%$,
whereas the overhead of the other data structures is between $\approx$$120$-$400\%$.

\subsection{Additional Experiments}

\begin{figure}
\includegraphics[width=0.35\textwidth]{experiments/macrobench/exp1_macrobench_throughput_exp_theta_0_5.png}

\includegraphics[width=0.35\textwidth]{experiments/macrobench/exp1_macrobench_throughput_exp_theta_0_9.png}

\includegraphics[scale=0.3]{experiments/macrobench/exp1_macrobench_throughput_legend.png}
\caption{YCSB database performance with different index data structures, and a skewed \textit{key access pattern}. (NM omitted because it is slower than BCCO.)}
\label{fig:experiments:ycsb}
\end{figure}

\paratitle{No-SQL database workload}
We study a simple \textit{in-memory database management system} called DBx1000~\cite{dbx1000},
which is used in multi-core database research. DBx implements a simple relational database,
which contains one or more \textit{tables}.
%, each of which consists of a sequence of \textit{rows}.
%It offers a variety of different concurrency control mechanisms for allowing processes to
%access tables and rows. We use its 2-phased locking option, which locks individual rows of
%tables, and has been shown to scale on simulated systems containing up to one thousand
%cores~\cite{dbx1000}.
Each table can have one or more \textit{key fields} and associated \textit{indexes}. Each index
allows processes to query a specific key field, quickly locating any rows in which the key field
contains a desired value. We replace the default index implementation in DBx with each of the
BSTs that we study.

Following the approaches in~\cite{dbx1000, ArbelRaviv2018GettingTT}, we run a subset of the well
known Yahoo! Cloud Serving Benchmark (YCSB) core with a single table containing 100 million
rows, and a single index. Each thread performs a fixed number of transactions (100,000 in our
runs), and the execution terminates when the first thread finishes performing its transactions.
Each transaction accesses 16 different rows in the table, which are determined by index lookups
on randomly generated keys. Each row is read with probability 0.9 and written with probability
0.1. The keys that a transaction will \textit{access} are generated according to a
\textbf{Zipfian} distribution %($\theta=0.6$ and $\theta=0.9$) 
following the approach in~\cite{Gray:1994}.

The results in Figure~\ref{fig:experiments:ycsb} show how performance
degrades as the distribution of \textit{accesses} to keys becomes highly skewed. (Higher
$\theta$ values imply a more extreme skew. A $\theta$ value of 0.9 is \textit{extremely}
skewed.)

\paratitle{Trees containing Zipfian-distributed keys} Since the performance of the ISTree can
theoretically degrade when the tree contains a highly skewed set of keys, we construct a
synthetic benchmark to study such scenarios. In this benchmark, $n$ threads access a single
instance of the ISTree, and there is a \textit{prefilling} phase followed by a \textit{measured}
phase. In the prefilling phase, each thread repeatedly generates a key from a Zipfian
distribution ($\theta=0.5$) over the key range $[1, 10^8]$ (picking one of 100 million
\textit{possible} keys), and inserts this key into the data structure (if it is not already
present). This continues until the data structure contains 10 million keys (only 10\% of the key
range), at which point the prefilling phase ends. In the measured phase, all threads perform
$u$\% updates and ($100-u$)\% searches (for $u \in \{0, 1, 10\}$) on keys drawn from the same
Zipfian distribution, for 30 seconds. This entire process is repeated for multiple trials, and
for thread counts $n \in \{24, 48, 96, 144, 190\}$ (with at least one core left idle to run
system processes).
%
\begin{figure}
\includegraphics[width=0.35\textwidth]{experiments/zipf/exp9_zipf_throughput_exp_u_0p,_k_2x10_8.png}

\includegraphics[width=0.35\textwidth]{experiments/zipf/exp9_zipf_throughput_exp_u_1p,_k_2x10_8.png}

\includegraphics[width=0.35\textwidth]{experiments/zipf/exp9_zipf_throughput_exp_u_10p,_k_2x10_8.png}

\includegraphics[scale=0.3]{experiments/zipf/exp9_zipf_throughput_legend.png}
\caption{Synthetic benchmark in which the \textit{set of keys stored} in a data structure is highly skewed.}
\label{fig:experiments:zipf}
\end{figure}
%
The results in Figure~\ref{fig:experiments:zipf} suggest that the ISTree
can remain robust even in scenarios where it contains a highly skewed distribution.

\paratitle{Artifact Evaluation}
All code is publicly available, and a working artifact is submitted as part of this work.

==> parts/intro.tex <==
% !TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

Efficient search data structures are critical in practical settings such as databases, 
where the large amounts of underlying data are usually paired 
with high search volumes, and with high amounts
of concurrency on the hardware side, via tens or even hundreds of parallel threads.
Consequently, there has been a significant amount of research on efficient
\emph{concurrent} implementations of search data structures.

For search data structures supporting predecessor queries,
which are the focus of this work, such as binary search trees (BSTs)
or balanced search trees, efficient implementations have been well researched
and are relatively well understood,
e.g.~\cite{BrownPhD, Natarajan:2014, Drachsler, Braginsky2012}.
However, these classic search data structures are subject
to the fundamental \emph{logarithmic} complexity thresholds (in the number of keys $n$),
even in the average case, which limits their performance for large key sets,
in the order of millions or even billions of keys.
In the sequential case, elegant and non-trivial techniques have been proposed
to reduce average-case complexity, by leveraging properties of the key space,
or of the key distribution. With one notable exception~\cite{SkipTrie},
these techniques are significantly less well understood for concurrent implementations.

This paper revisits this area,
and provides the first efficient, non-blocking concurrent implementation
of an \emph{interpolation search tree} data structure~\cite{IST}, called the C-IST.
The C-IST is \emph{dynamic}, in that it supports concurrent searches,
insertions and deletions.
Interpolation search trees, presented in the next section,
have amortized worst-case $O( \log n)$ time for standard operations,
but achieve $O( \log \log n )$ expected amortized time complexity for insert and delete,
and $O( \log \log n)$ expected time for search,
by leveraging smoothness properties
of the key distribution~\cite{IST}.
Our concurrent implementation preserves these properties with high probability.

To ensure correctness, non-blocking progress, and scalability in the concurrent setting,
we introduce several new techniques relative to sequential ISTs.
Specifically, our contributions are as follows:

\begin{itemize}
\item
We describe the first non-blocking concurrent interpolation search tree (C-IST)
based on atomic compare-and-swap (CAS) instructions
(Section \ref{sec:algorithm}), with expected lookup time $O( \log \log n + p)$,
and expected amortized $O( \log \log n + p)$ time for insert and delete.
\item
We design a \emph{parallel}, \emph{non-blocking} rebuilding algorithm
to provide fast and scalable periodic rebuilding for C-ISTs
(Section \ref{sec:concurrent-collaborative-rebuild}). 
We believe that this technique is applicable to other concurrent data structures
that require rebuilding.
\item
We prove the correctness, non-blocking and complexity properties of the C-IST
(Section \ref{sec:analysis}).
\item
We provide a C-IST implementation in C++, and  compare its performance against
concurrent $(a,b)$-trees~\cite{BrownPhD},
Natarajan and Mittal's concurrent BSTs~\cite{Natarajan:2014},
and Bronson's concurrent AVL trees~\cite{bronsonavl} (Section \ref{sec:evaluation}).
We report performance improvements of $15\%-50\%$
compared to $(a,b)$-trees (the best-performing current alternative) on large datasets,
and improvements of up to $3.5\times$ compared to the other concurrent trees,
depending on the proportion of updates.
We also analyze the average depth and cache-miss behavior,
present a breakdown of the execution time,
show the impact of the parallel rebuilding algorithm,
and compare memory footprints.
\end{itemize}

\iffalse

\dan{just an outline, feel free to ignore}

\begin{itemize}
  \item There has been a tremendous amount of research studying efficient concurrent search data structures. 
  We now have a good understanding of BSTs, as well as balanced search trees. 
  \item However, in the sequential case, there are several non-trivial techniques which circumvent the logarithmic bound without rebalancing, for example by making assumptions on the key distribution. 
  \item These techniques are less well understood in the context of concurrency, with the SkipTrie being the only known proposal in this space. 
  \item This paper revisits these techniques, and provides the first concurrent implementation of a dynamic interpolation search tree. 
  The implementation guarantees logarithmic amortized worst-case bounds w.h.p., and $O( \log \log n )$ amortized cost for all operations \dan{again, fix the contention factor!} under distributional assumptions. 
  \item New techniques. 
  \item Cover the experimental results. 
\end{itemize}
\fi


==> parts/old-evaluation.tex <==
% !TEX root = ../main.tex

\section{Evaluation}
\label{sec:evaluation}

We implemented the concurrent IST in C++,
and compared it against several state of the art concurrent data structures.
We ran the benchmarks
on a NUMA system with four Intel Xeon Gold 6150 3.7GHz CPUs,
each of which has 18 cores and 36 hardware threads.
Within each CPU, cores share a 24.75MB LLC,
and cores on different CPUs do not share any caches.
The system has 512GB of RAM,
and runs Debian Linux 4.9.82-1 with kernel 4.9.0-6.
Our code was compiled with GCC 6.3.0-18,
with the highest optimization level (\texttt{-O3}).
Threads were \textit{pinned} to cores such that
thread counts up to 36 ran on only one CPU,
thread counts up to 72 run on only two CPUs,
and so on.
We used the fast scalable allocator jemalloc 5.0.1-25.
When a page of memory is allocated on our four-processor Xeon system,
it has an \textit{affinity} for a single CPU,
and other CPUs pay a penalty to access it.
We therefore used the \texttt{numactl --interleave=all} option to ensure
that pages are evenly distributed across CPUs.
We compared our IST implementation to the leading non-blocking binary search tree (BST)
due to Natarajan and Mittal~\cite{Natarajan:2014}
and a fast non-blocking $(a,b)$-tree (ABTREE) due to Brown~\cite{BrownPhD},
which is a concurrency-friendly variant of a B-tree.


\subsection{Lookup}

We implemented a synthetic microbenchmark
in which $n$ threads access a single shared data structure.
%repeatedly perform \textit{lookups} in a single shared data structure.
We used different thread counts
($1$, $18$, $36$, $72$, $108$ and $144$)
and tree sizes
(1 million, 10 million, 100 million and 1 \textit{billion} keys).
For each data structure, thread count and tree size, we ran five timed \textit{trials}.
In each trial,
the desired number of keys was inserted into the data structure.
Then, for 10 seconds,
all threads repeatedly performed lookups
on randomly chosen keys,
so that there is a $50\%$ probability of finding the key.

\paratitle{Results}
We show the results in Figure~\ref{fig:bench-lookup-comparison-cpp},
where we plot the total number of lookups per microsecond versus the number of threads,
for each tree size.
Variance was very low at each data point, less than 1\% of the mean.
The results show a substantial performance advantage of the IST:
up to $2\times$ speedup compared to the ABTREE,
and $5\times$ compared to the BST.

\begin{figure}[t]
\small

%  \begin{center}
%    \begin{tikzpicture}
%      \node at (0,0) [
%      minimum width=1.5mm,
%      minimum height=1.5mm,
%      fill={rgb:red,1;green,4;blue,5},
%      ] {};
%    \end{tikzpicture}
%    BST
%    \quad
%    \begin{tikzpicture}
%      \node at (0,0) [
%      minimum width=1.5mm,
%      minimum height=1.5mm,
%      fill={rgb:red,1;green,3;blue,1},
%      postaction={
%      pattern color=white,
%      pattern=north east lines,
%      },
%      ] {};
%    \end{tikzpicture}
%    AB tree
%    \quad
%    \begin{tikzpicture}
%      \node at (0,0) [
%      minimum width=1.5mm,
%      minimum height=1.5mm,
%      fill={rgb:red,5;green,1;blue,1},
%      postaction={
%      pattern color=white,
%      pattern=north west lines,
%      },
%      ] {};
%    \end{tikzpicture}
%    IST
%  \end{center}

  \centering

  \makebox[0.4\linewidth]{\textbf{1 million key set}}
  \makebox[0.4\linewidth]{\textbf{10 million key set}}
  
  \includegraphics[width=0.48\linewidth]{experiments/xeon-gold-6150-x4/line_2m.PNG}
  \includegraphics[width=0.48\linewidth]{experiments/xeon-gold-6150-x4/line_20m.PNG}
  
  \makebox[0.4\linewidth]{\textbf{100 million key set}}
  \makebox[0.4\linewidth]{\textbf{1 billion key set}}

  \includegraphics[width=0.48\linewidth]{experiments/xeon-gold-6150-x4/line_200m.PNG}
  \includegraphics[width=0.48\linewidth]{experiments/xeon-gold-6150-x4/line_2b.PNG}
  
  \vspace{1mm}
  \includegraphics[width=0.3\linewidth]{experiments/xeon-gold-6150-x4/legend.PNG}
  % \input{experiments/lookup-cpp}
  \vspace{-3mm}
  \caption{Lookup Comparison with Similar Data Structures (C++, Xeon Gold 6150)}
  \label{fig:bench-lookup-comparison-cpp}
\end{figure}

Interestingly, IST is much faster in the case where the trees contain 1 million keys,
but less compared to the ABTREE with 10 million keys,
and then gradually regains its advantage as the trees grow larger.
To explain this,
we used the C PAPI 5.4.1.0 library
to measure the number of LLC misses for each data structure and size.
Figure~\ref{fig:bench-cpp-l3misses} summarizes the results.

\begin{figure}
  \small
  \centering
  \begin{center}
    \begin{tikzpicture}
      \node at (0,0) [
      minimum width=1.5mm,
      minimum height=1.5mm,
      fill={rgb:red,1;green,4;blue,5},
      ] {};
    \end{tikzpicture}
    IST
    \quad
    \begin{tikzpicture}
      \node at (0,0) [
      minimum width=1.5mm,
      minimum height=1.5mm,
      fill={rgb:red,1;green,3;blue,1},
      postaction={
      pattern color=white,
      pattern=north east lines,
      },
      ] {};
    \end{tikzpicture}
    ABTREE
    \quad
    \begin{tikzpicture}
      \node at (0,0) [
      minimum width=1.5mm,
      minimum height=1.5mm,
      fill={rgb:red,5;green,1;blue,1},
      postaction={
      pattern color=white,
      pattern=north west lines,
      },
      ] {};
    \end{tikzpicture}
    BST
    %\quad
    %\begin{tikzpicture}
    %\node at (0,0) [
    %  minimum width=1.5mm,
    %  minimum height=1.5mm,
    %  fill={rgb:red,5;green,1;blue,3},
    %  postaction={
    %    pattern color=white,
    %    pattern=crosshatch,
    %  },
    %] {};
    %\end{tikzpicture}
    %SkipTrie
  \end{center}
% \includegraphics[width=\linewidth]{experiments/xeon-gold-6150-x4/l3misses.PNG}
  \input{experiments/xeon-gold-6150-x4/llc.tex}
  \vspace{-3mm}
  \caption{Comparison of LLC misses per lookup (C++, Xeon Gold 6150)}
  \label{fig:bench-cpp-l3misses}
\end{figure}

With 1 million keys,
IST fits almost entirely in cache, incurring only 0.09 LLC misses per lookup,
while ABTREE incurs 1.5 misses per lookup,
and BST incurs 3.5 misses per lookup.
IST has such a large advantage in this case
because it almost never accesses main memory.
With 10 million keys,
IST no longer fits in cache,
and IST and ABTREE have a similar number of LLC misses per lookup
(6.0 vs. 6.6).
However, as the number of keys continues to grow,
the number of LLC misses incurred per lookup increases much more slowly for the IST,
than for the ABTREE and the BST.
In the 1 billion key case, the IST incurs only 13.1 misses per lookup,
compared to 19.0 for the ABTREE, and 33.2 for the BST.


\subsection{Insert and remove}

TODO: Add the evaluation of concurrent rebuilding.


\subsection{Approximate counters}

TODO: Add the evaluation of C-IST without approximate counters.


==> parts/title.tex <==
% !TEX root = ../main.tex

%% Title information
\title[Non-Blocking Interpolation Search Trees]{Non-Blocking Interpolation Search Trees with Doubly-Logarithmic Running Time}         %% [Short Title] is optional;
                                        %% when present, will be used in
                                        %% header instead of Full Title.
%\titlenote{with title note}             %% \titlenote is optional;
                                        %% can be repeated if necessary;
                                        %% contents suppressed with 'anonymous'
%\subtitle{Subtitle}                     %% \subtitle is optional
%\subtitlenote{with subtitle note}       %% \subtitlenote is optional;
                                        %% can be repeated if necessary;
                                        %% contents suppressed with 'anonymous'


%% Author information
%% Contents and number of authors suppressed with 'anonymous'.
%% Each author should be introduced by \author, followed by
%% \authornote (optional), \orcid (optional), \affiliation, and
%% \email.
%% An author may have multiple affiliations and/or emails; repeat the
%% appropriate command.
%% Many elements are not rendered, but should be provided for metadata
%% extraction tools.

%% Author with single affiliation.
\author{Trevor Brown}
%\authornote{with author1 note}          %% \authornote is optional;
                                        %% can be repeated if necessary
%\orcid{nnnn-nnnn-nnnn-nnnn}             %% \orcid is optional
\affiliation{
  % \position{Position1}
  % \department{Department1}              %% \department is recommended
  \institution{University of Waterloo}            %% \institution is required
  % \streetaddress{Street1 Address1}
  % \city{City1}
  % \state{State1}
  % \postcode{Post-Code1}
  \country{Canada}                    %% \country is recommended
}
\email{me@tbrown.pro}          %% \email is recommended

%% Author with two affiliations and emails.
\author{Aleksandar Prokopec}
%\authornote{with author2 note}          %% \authornote is optional;
                                        %% can be repeated if necessary
\orcid{0000-0003-0260-2729}             %% \orcid is optional
\affiliation{
  %\position{Position2a}
  %\department{Department2a}             %% \department is recommended
  \institution{Oracle Labs}           %% \institution is required
  % \streetaddress{Street2a Address2a}
  % \city{City2a}
  % \state{State2a}
  % \postcode{Post-Code2a}
  \country{Switzerland}                   %% \country is recommended
}
\email{aleksandar.prokopec@gmail.com}         %% \email is recommended


%% Author with single affiliation.
\author{Dan Alistarh}
%\authornote{with author1 note}          %% \authornote is optional;
                                        %% can be repeated if necessary
\orcid{0000-0003-3650-940X}             %% \orcid is optional
\affiliation{
  % \position{Position1}
  % \department{Department1}              %% \department is recommended
  \institution{Institute of Science and Technology}            %% \institution is required
  % \streetaddress{Street1 Address1}
  % \city{City1}
  % \state{State1}
  % \postcode{Post-Code1}
  \country{Austria}                    %% \country is recommended
}
\email{dan.alistarh@ist.ac.at}          %% \email is recommended


%% 2012 ACM Computing Classification System (CSS) concepts
%% Generate at 'http://dl.acm.org/ccs/ccs.cfm'.
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003752.10003809.10011778</concept_id>
<concept_desc>Theory of computation~Concurrent algorithms</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10003809.10010170.10010171</concept_id>
<concept_desc>Theory of computation~Shared memory algorithms</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10011777.10011778</concept_id>
<concept_desc>Computing methodologies~Concurrent algorithms</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Theory of computation~Concurrent algorithms}
\ccsdesc[300]{Theory of computation~Shared memory algorithms}
\ccsdesc[500]{Computing methodologies~Concurrent algorithms}

%% End of generated code


%% Keywords
%% comma separated list
\keywords{concurrent data structures, search trees, interpolation, non-blocking algorithms}

